Anomaly Inflow, Accidental Symmetry, and Spontaneous Symmetry Breaking

We consider the 6d (1,0) SCFT on a stack of $N$ M5-branes probing a $\mathbb C^2/\mathbb Z_2$ singularity. In particular, we study its compactifications to four dimensions on a smooth genus-$g$ Riemann surface with non-trivial flavor flux, yielding a family of 4d CFTs. By tracking the M-theory origin of the global symmetries of the 4d CFTs, we detect the emergence of an accidental symmetry and the spontaneous symmetry breaking of a $U(1)$ generator. These effects are visible from geometric considerations and not apparent from the point of view of the compactification of the 6d field theory. These phenomena leave an imprint on the 't Hooft anomaly polynomial of the 4d CFTs, which is obtained from recently developed anomaly inflow methods in M-theory. In the large-$N$ limit, we identify the gravity dual of the 4d setups to be a class of smooth $AdS_5$ solutions first discussed by Gauntlett-Martelli-Sparks-Waldram. Using our anomaly polynomial, we compute the conformal central charge and a non-Abelian flavor central charge at large $N$, finding agreement with the holographic predictions.

==> sec_setup.tex <==
%!TEX root = ./GMSWmain.tex

\section{Six-dimensional setup}

The main setup of interest is a stack of $N$ M5-branes probing a $\mathbb{C}^2/\mathbb{Z}_2$ orbifold singularity in M-theory.  First, we discuss some general aspects where the M5-branes are probing a $\mathbb{C}^2/\mathbb{Z}_k$ orbifold fixed point.

\subsection{Aspects of M-theory on $\mathbb{C}^2/\mathbb{Z}_k$}

First we consider the M-theory background with the orbifold $\mathbb{C}^2/\mathbb{Z}_k$.  Let $(x^0,\cdots,x^5)$ be the coordinates along an $\mathbb{R}^6$ plane, and $(y^1,\cdots,y^5)$ be the coordinates along the transverse directions.  The latter parametrize a five-dimensional space $\mathbb{C}^2 \times \mathbb{R}$ with complex coordinates $(z_1= y^1+ i y^2, z_2 = y^3+iy^4)$.  The orbifold action is 
\begin{equation}
(z_1,z_2, y^5) \sim (e^{\frac{2\pi i}k} z_1,e^{-\frac{2\pi i}k}z_2, y^5).  
\end{equation} A local metric for the M-theory background is given as
\begin{align}
ds^2_{11} &= ds^2(\mathbb{R}^6) +  dr^2 + r^2 \, ds^2 (S^4/\mathbb{Z}_k)   \label{kbackground} \\
ds^2 (S^4/\mathbb{Z}_k)  &= \frac{d\mu^2}{1-\mu^2} + (1-\mu^2) \left[ \frac{1}{k^2} \,
D\varphi^2 + \frac{1}{4} \, ds^2(S^2_\psi) \right], \label{sphereorb}\\
ds^2(S^2_\psi) &= d\theta^2 + \sin^2 \theta \,   d\psi^2, \qquad D\varphi = d\varphi + \frac{k}{2} \cos \theta \,  d\psi.  
\end{align} The radius $r$ is constructed from $y^5$ and the radii of the two complex planes, in particular we have $y^5 = r \mu$.  The circle coordinates have periodicity $(\Delta \psi = 2\pi, \Delta \varphi = 2\pi)$.  For $k=1$, the metric \eqref{sphereorb} is that of round four-sphere.  When $k> 1$, the orbifold action admits two $\mathbb{R}^4/\mathbb{Z}_{k}$ fixed points at the poles of the sphere at $\mu = \pm 1$.  At constant values of $\mu$, the three dimensional sections of the four-sphere are $S^1_{\phi}$ bundles over $S^2_\psi$ with degree $k$.  The isometries of $S^1_\varphi$ and $S^2_\psi$ lead to a $U(1)_\varphi \times SU(2)_\psi$ gauge symmetry on the extended seven-dimensional directions of the M-theory background.  This is the subgroup of the $SO(5)$ isometry of the sphere preserved by the orbifold action.  

The region near an orbifold fixed point of the sphere corresponds to a single center Taub-NUT space, the metric near each pole is 
\begin{equation}
ds^2  \cong \frac{1}{V} \,  D\varphi^2 + V \,  \left[d R^2 + R^2 \,  ds^2(S^2_\psi) \right], \quad V = \frac{k}{2R}, \quad R = \frac{1}{k}  \, (1\mp \mu), \quad \mbox{for} \quad \mu = \pm 1. \label{polesmetric}
\end{equation} The orbifold singularities can be resolved locally by replacing the single center Taub-NUT space to a Gibbons-Hawking space with $k$ sources of unit charge.  Such spaces are $S^1_\varphi$ bundles over $\mathbb{R}^3$ with metric given as 
\begin{equation}
ds^2 = V^{-1} \left(d\varphi + A \right)^2  + V \left(dX^2 + dY^2 + dZ^2\right), \quad \mbox{with} \quad d V = \star_{\mathbb R^3} dA \ ,
\end{equation} where $V$ is a potential on the 3D base space and $A$ is a connection one-form for the circle bundle.  The potential satisfies Laplace's equation on the $\mathbb{R}^3$ base.  A general solution of Gibbons-Hawking space is given by inserting $k$ centers at positions $\vec{X}_I = (X_I,Y_I,Z_I)$ with charge $n^I$.  The potential is
\begin{equation}
V = v_0 + \frac{1}{2} \sum_I \frac{n^I}{ \big |\vec{X} -\vec{X}_I  \big |}.
\end{equation} The parameter $v_0$ fixes the asymptotic size of the circle.  The coordinate $\varphi$ has period $2\pi$.  The space is Asymptotically Locally Flat (ALF) when $v_0\neq 0$ with topology of $S^1 \times \mathbb{R}^3$, and asymptotically Locally Euclidean (ALE) when $v_0 =0$ with topology of $\mathbb{R}^4$.

The region near each center is described by a $\mathbb{R}^4/\mathbb{Z}_{n^I}$ orbifold fixed point where $S^1_\varphi$ shrinks.  A two-cycle can be obtained by taking $S^1_\varphi$ with a segment on $\mathbb{R}^3$ that connects two singularities.  There are $k-1$ independent two-cycles with harmonic representatives, $\omega^i$ $(i\in \{1,\cdots, k-1\})$.  When all $n^I=1$, the space is smooth with $k-1$ two-cycles.  This corresponds to a resolution of the orbifold singularity.  The $S^1_\psi$ circle of $S^2_\psi$ in \ref{polesmetric}, is identified with the rotation on the $(X,Y)$ plane.  Resolving the singularity breaks the $SU(2)_\psi$ isometry of $S^2_\psi$ to a $U(1)_\psi$ corresponding to the rotations of $S^1_\psi$.  

M-theory, in the supergravity limit, can be studied on the space \eqref{kbackground} where we replace the two orbifold singularities with their smooth resolutions.  This local deformation is always possible since the asymptotic space of Gibbons-Hawking is fixed by the total charge.  M-theory has a 2-form gauge symmetry with a 3-form potential, $C_3$.  There are massless fluctuations of the $C_3$ potential on the extended seven-dimensional space coming from the resolutions of the singularities.  In reducing M-theory on the compact space, we can add terms to $C_3$ as 
\begin{equation}
C_3 = a_{ i}^\mathrm N \wedge \omega^i_{\mathrm N} 
+  a_{ i}^\mathrm S \wedge \omega^i _{\mathrm S}+ \cdots \label{C36d}
\end{equation} where $(\omega_\mathrm N^i,\omega_\mathrm S^i)$ are the resolution harmonic two-forms for the north and south singularities, respectively.  The one-forms $(a^\mathrm N_i,a^\mathrm S_i)$ are massless gauge field on the seven-dimensional space.  Each orbifold fixed point leads to a $U(1)^{k-1}$ gauge symmetry in M-theory which enhances to an $SU(k)$ gauge symmetry in the singular limit \cite{Sen:1997kz}.  To summarize, the M-theory background admits an $SU(2)_\psi \times SU(k)_\mathrm N \times SU(k)_\mathrm S \times U(1)_\varphi$ bosonic gauge symmetry.  
 

We are interested in the field theory that describe the low energy dynamics of a stack of $N$ M5-branes probing the M-theory singularity at $r=0$ in \eqref{kbackground}.  The gauge symmetry of the M-theory background induces a global symmetry on the worldvolume directions of the M5-branes.  The $SU(2)_\psi$ symmetry from $S^2_\psi$ corresponds to an $SU(2)_\mathcal{R}$ R-symmetry, whiles the rest $SU(k)_\mathrm N \times SU(k)_\mathrm S \times U(1)_\varphi$ imprints as a flavor symmetry. In particular,
the 7d gauge fields $(a^\mathrm N_i , a^\mathrm S_i)$
yield 6d background connections $(A^\mathrm N_{6d \, i} , A^\mathrm S_{6d \, i})$. This configuration preserves eight supercharges leading to a six-dimensional superconformal field theory with a $(1,0)$ supersymmetry 
 \cite{Brunner:1997gk,Blum:1997fw,Blum:1997mm,Intriligator:1997dh,Brunner:1997gf,Hanany:1997gh}.  

\subsection{The case   $k=2$}\label{k2res}

The resolution space of $S^4/\mathbb{Z}_2$ has an enhanced symmetry.  The $U(1)_\varphi$ isometry of $S^1_\varphi$ in $S^4/\mathbb{Z}_2$
enhances  to an $SU(2)_\varphi$ isometry group as can be seen by rewriting the metric as
\begin{equation}
ds^2(S^4/\mathbb{Z}_2) = \frac{d\mu^2}{1-\mu^2} + \frac{1}{4} \,  (1-\mu^2) \,  \left[ 
D\psi^2 + d\theta^2 + \sin^2 \theta  \,  d\varphi^2 \right] , \quad  D\psi = d\psi + \cos \theta  \,  d\psi. \label{sphere2}
\end{equation}  The resolution of the orbifold singularities at $\mu = \pm 1$ preserve the isometries of $S^2_\varphi$ composed of $(\theta, \psi)$ in the metric of $S^4/\mathbb{Z}_2$ above.  This follows from the fact that the resolution space of $\mathbb{R}^4/\mathbb{Z}_2$ is the Eguchi-Hanson space \cite{Eguchi:1978xp}.  To see this more explicitly, write the potentials for the two center Gibbons-Hawking space with unit charge as
\begin{align}
V &= \frac{1}{2 R_+} + \frac{1}{2 R_-}, \qquad A = \frac{1}{2} \left(\frac{Z_+}{R_+} + \frac{Z_-}{R_-} \right) d \tan^{-1} \left(Y/X \right)  \ , \\
R_\pm^2 &= X^2 + Y^2 + Z_\pm^2 \ , \qquad  Z_\pm = Z \pm Z_0 \ .   
\end{align} The centers are sitting at $(0,0,\pm Z_0)$.  The metric of the resolved space can be written as 
\begin{equation}
ds^2 = \frac{R^4}{R^4-a^4} \, dR^2 + \frac{R^2}{4} \,  \left[d\theta^2 + \sin^2 \theta \,
 d\varphi^2 + \frac{R^4-a^4}{R^4} \left(d\psi + \cos \theta \, d\varphi \right)^2 \right]  \ ,\label{EHspace}
\end{equation} where we have made the coordinate transformation \cite{Prasad:1979kg}
\begin{equation}
Z=\frac{R^2}{4} \, \cos \theta \  , \quad 
X = \frac{\sqrt{R^4-a^4}}{4}\,  \sin \theta  \,  \cos \psi \  , \quad 
Y = \frac{\sqrt{R^4-a^4}}{4} \, \sin \theta  \,  \sin \psi \ .
\end{equation}  
 The space smoothly caps off at $R=a$ where the $S^1_\psi$ circle shrinks.  The two-sphere, $S^2_\varphi$, composed of $(\theta, \varphi)$ in the resolved space has a finite size of $a/2$ at $R=a$.  The two-sphere in this region also corresponds to the two-cycle of the resolution of the $\mathbb{R}^4/\mathbb{Z}_2$.  

The singularities of $S^4/\mathbb{Z}_2$ are resolved by excising the singular region and gluing in the Eguchi-Hanson space describe in \eqref{EHspace}.  The $S^2_\varphi$ of \eqref{EHspace} is identified with the $S^2_\varphi$ of $S^4/\mathbb{Z}_2$ in \eqref{sphere2}.  In this sense, the resolution of the singularities on the sphere preserves its isometries.  

The smooth geometry obtained from the resolution of $S^4/\mathbb{Z}_2$ is denoted as $M_4$.  It has the topology of $S^2 \times S^2$ and corresponds to the Hirzebruch surface $\mathbb{F}_2$.  It is useful to write a local metric for the space $M_4$,
\begin{align}
ds^2(M_4) =  h_1(\mu) \, ds^2(S^2_\varphi) 
+ h_2(\mu) \,  d\mu^2 
+  h_3(\mu)  \, D\psi^2 \  , \qquad 
D\psi &= d\psi + \cos \theta  \,  d\varphi \  . \label{M4metric}
\end{align} The coordinate $\mu$ takes value in the interval $[\mu_\mathrm S, \mu_\mathrm N]$.  The boundary conditions of the $h$'s are fixed by regularity of the metric at the bounds, and in particular, $h_3$ must vanish on them.  The two-sphere $S^2_\varphi$ is not shrinking at the north and south poles of $M_4$ where the $S^1_\psi$ is shrinking.  The two-spheres at the tip of the $\mu$-interval correspond to two-cycles denoted as $(\mathcal{S}^2_\mathrm S, \mathcal{S}^2_\mathrm N)$ respectively.  The volume of these cycles are then $(h_1(\mu_\mathrm S),h_1(\mu_\mathrm N))$ respectively.  

%The singular metric in \eqref{sphere2} is recovered when
%\begin{equation}
%h_1^{-1}(\mu)  = h_2(\mu) = h_3(\mu) = 1-\mu^2, \qquad \mbox{and} \qquad a_N = a_S =1. 
%\end{equation} 

The sizes of the two-cycles $(\mathcal{S}^2_\mathrm S, \mathcal{S}^2_\mathrm N)$ are moduli parameters of $M_4$.  In the singular limit where they vanish, $M_4 \to S^4/\mathbb{Z}_2$.  The four-sphere admits a left $SU(2)$ and a right $SU(2)$ action; these are preserved by the $\mathbb{Z}_2$ orbifold action, and are related to the isometries of $SU(2)_\psi \times SU(2)_\varphi$ rotations.  
The $U(1)_\psi \times SU(2)_\varphi$ are manifest as isometries of $S^1_\psi \times S^2_\varphi$ of the metric \eqref{sphere2}.  The total gauge symmetry in seven dimensions is $SU(2)_\psi \times SU(2)_\varphi \times
SU(2)_\mathrm N \times SU(2)_\mathrm S$. 
%It induces an $SU_N(2) \times SU_S(2)\times SU_\varphi(2)$ flavor symmetry and $SU_\mathcal{R}(2)$ R-symmetry on the worldvolume of the branes.  




\paragraph{Anomalies of the 6d setup}

Anomaly inflow for flat M5-branes probing orbifold singularities was studied in \cite{Ohmori:2014kda}.
See also \cite{toappear} for a review of the computation.
The inflow computation yields an 8-form $I_8^{\rm inflow}$
which captures the variation of the M-theory action in the 
presence of the M5-brane stack. 
The inflow anomaly polynomial
counterbalances the anomalies of the worldvolume degrees of freedom,
which at low energies consists of an interacting SCFT
and of modes that decouple in the IR,
\beq
I_8^{\rm inflow} + I_8^{\rm SCFT} + I_8^{\rm decoupl} = 0 \ .
\eeq
The inflow anomaly polynomial reads
\begin{align} 
- I_8^{\rm inflow} & = 
 \frac{N^3 }{6} \, \big[ c_2^\varphi - c_2^\psi  \big]^2 
 +  \frac{N }{12}  \, 
 \big[ 4 \, c_2^\varphi
- 3 \, c_2^\psi \big] \, c_2^\psi 
+ \frac{N}{24} \, 
 \big[ 2 \, c_2^\varphi
-  \, c_2^\psi \big] \, p_1(TW_6)
\nn \\
&- \frac{1}{32 \, N} \, 
\bigg[ 
  \frac{ {\rm tr} \, (F_{6d}^{\rm N})^2}{(2\pi)^2}
-  \frac{{\rm tr} \, (F_{6d}^{\rm S})^2}{(2\pi)^2}
\bigg] ^2
   + \frac{N }{4} \, 
\big[ c_2^\varphi - c_2^\psi  \big] \, \bigg[ 
  \frac{ {\rm tr} \, (F_{6d}^{\rm N})^2}{(2\pi)^2}
+  \frac{{\rm tr} \, (F_{6d}^{\rm S})^2}{(2\pi)^2}
\bigg]
\nn \\
&  +  
 \frac{N}{192} \big[  p_1(TW_6)^2 - 4 \, p_2(TW_6)  \big]
 \ .  
\end{align}
We have introduced the compact notation
\beq
c_2^\varphi \equiv c_2(SU(2)_\varphi) \ , \qquad
c_2^\psi \equiv c_2(SU(2)_\psi)  \ .
\eeq
The anomaly of the decoupling modes is given by
\begin{align}
I_8^{\rm decoupl} & = 
 I^{\rm tensor}_8 + \frac 12 \,  I_8^{\rm vec, N}
+ \frac 12 \,  I_8^{\rm vec, S} \ .
\end{align}
The 8-form $ I^{\rm tensor}_8$ is the anomaly polynomial
of a   6d (1,0) tensor multiplet,
\beq
I_8^{\rm tensor} = 
\frac{1}{24} \,( c_2^\psi)^2 + \frac{1}{48} \, c_2^\psi \, p_1(TW_6)
+ \frac{23}{5760} \, p_1(TW_6)^2
- \frac{29}{1440} \, p_2(TW_6) \ .
\eeq
The 8-form $I_8^{\rm vec, N}$ is the anomaly polynomial
of a   6d (1,0) vector multiplet of $SU(2)_\mathrm N$,
\begin{align}
I_8^{\rm vec,N} & = - \frac 18 \, (c_2^\psi)^2
- \frac{1}{16} \, c_2^\psi \, p_1(TW_6)
- \frac{1}{1920} \big[  7 \, p_1(TW_6)^2 - 4 \, p_2(TW_6) \big]
\nn \\
& - \frac 12 \, c_2^\psi \, \frac{{\rm tr}  \, (F_{6d}^N)^2}{(2\pi)^2}
- \frac{1}{24} \, p_1(TW_6) \,   \frac{{\rm tr}  \, (F_{6d}^N)^2}{(2\pi)^2}
- \frac {1}{12} \, \bigg[    \frac{{\rm tr} \, (F_{6d}^N)^2}{(2\pi)^2}\bigg]^2  \ .
\end{align}
The quantity $I_8^{\rm vec, S}$  is completely analogous.\footnote{The
trace `tr' is normalized in such a way that,
if $n_{1,2}$ are the Chern roots of an $SU(2)$ bundle  with $n_1 + n_2 = 0$,
then 
${\rm tr} F^2 /(2\pi)^2 = - 2 \, (n_1^2 + n_2^2)$.
}

 
%
%
%\begin{comment}
%In the reduction of M-theory onto the seven-dimensional space, the gauge fields for the global symmetry can be added to metric and to the $C_3$ potential.  In the supergravity analysis, the gauge field corresponding to the Cartan element of the $SU_\psi(2)$ R-symmetry can be turned by gauging the $U_\psi(1)$ action of $S^1_\psi$.  Similarly $SO(3)$ gauge fields for the $S^2_\varphi$ can also be add.  
%
%The gauging of the Cartan elements of $SU_N(2) \times SU_S(2)$ is obtained from the $C_3$ potential as
%\begin{equation}
%C_3 = A^N \omega_N + A^S \omega_S, \quad \mbox{with} \quad G_4 = F^N \omega_N + F^S \omega_S
%\end{equation} where $G_4 = d C_3$ is the four-form flux of M-theory.  The field strength for the $U(1)$ gauge fields $(A^S,A^N)$ are given as $(F^S,F^N)$, and the harmonic two-forms associated to the two-cycles $(\mathcal{S}^2_S, \mathcal{S}^2_N)$ are denoted as $(\omega_S, \omega_N)$.
%
%The gauging of the $U(1)$ subgroup of the $SU_\mathcal{R}(2)$ R-symmetry is obtained by adding a connection for the $S^1_\psi$ circle as
%\begin{align} 
%D\psi \, \to \, \tilde{D}\psi = d\psi + \cos(\theta) d\varphi - A^\psi, \quad \mbox{with} \quad F^\psi = dA^\psi.
%\end{align} The $SU(2)$ from the $S^2_\varphi$ is can be gauged by using embedding coordinated for the two-sphere, which are $(y^1 = \sin{\theta} \cos(\varphi), y^2 = \sin(\theta) \sin(\varphi), y^3 = \cos(\theta))$.  The gauged one-forms that characterize the sphere and the metric are given as
%\begin{equation}
%dy^a \, \to \, Dy^a = dy^a + A^{ab} y^c \delta_{bc}, \qquad ds^2(S^2_\varphi) = \delta_{ab} Dy^a Dy^b
%\end{equation} where $A^{bc}$ are the $SO(3)$ connection forms over the external spacetime of M-theory.  The gauge invariant volume form of the sphere and the field strength for the connections can be given as
%\begin{equation}
%D \Omega_2 =\frac{1}{2} \epsilon_{abc} Dy^a Dy^b y^c, \qquad F^{ab} = D A^{ab} = dA^{ab} + A^{ac} \wedge A^{cb} \delta_{ab}
%\end{equation} where $\epsilon_{abc}$ and $\delta_{ab}$ are the Levi-Civita tensor and identity metric of the embedding $\mathbb{R}^3$ space for the sphere.  These two objects can be added to yield a gauge invariant, closed, and globally define angular form for the sphere give as 
%\begin{equation}\label{e2svarphi}
%4\pi e_2 = D\Omega_2 + \epsilon_{abc} F^{ab} y^c, \quad \mbox{so that} \quad \int_{S^2_\varphi} e_2 =1.   
%\end{equation}  The gauge field for the Cartan $U(1)$ corresponding to $S^1_\varphi$ is given by $A^\varphi = A^{12}$.  The gauging for the $U(1)$ is given as
%\begin{equation}
%d\varphi \, \to \,  \tilde{D} \varphi = d\varphi - A^\varphi, \qquad F^\varphi = d A^\varphi.  
%\end{equation} 
%
%\end{comment} 
%
%\paragraph{$G_4$ flux for M5-brane system}
%
%We are interested in the SCFT that describe the low energy dynamics of a stack of $N$ M5-branes sitting at $r=0$ in the M-theory background given for \eqref{kbackground} for $k=2$.  In presence of the branes, the four-form flux $G_4$ admits a magnetic source
%\begin{equation}
%dG_4 = N \delta_{W_6}
%\end{equation} where $\delta_{W_6}$ is a five-form that localize on the worldvolume of the branes, $W_6$, at $r=0$.  This source imposes a boundary condition for $G_4$ in the region near the branes.  This can be characterized by introducing a bump function, $\rho(r)$, that vanish as $r\to \infty$ and approach $1$ in the region near the branes.  We can write
%\begin{equation}
%G_4 = 2\pi \rho(r) \overline {G}_4+ \dots , \quad \mbox{with} \quad \int_{M^4} \overline{G}_4 = N. \label{bd6d}
%\end{equation} The ellipses corresponds to terms that are not relevant in the region near the branes but are needed to for closure of $G_4$.  The boundary condition, $\overline{G}_4$, must be closed and can be written in terms of a normalized volume form of $M_4$, given as
%\begin{equation} \label{barG4_6d}
%\overline{G}_4 = 2 N V_4, \qquad V_4 = \frac{1}{2} \,  d\gamma(\mu) \wedge \frac{D \psi}{2\pi} \wedge V^\varphi_2 \ , \qquad \int_{M_4} V_4 = \frac{1}{2} \ .
%\end{equation}
%The function $\gamma(\mu)$ can be given in terms of the $h$'s above and it is normalized by the integration condition on $V_4$.  The volume form of $S^2_\varphi$ is given as $V_2^\varphi$,
%with the normalization $\int_{S^2_\varphi} V_2^\varphi = 1$.
%
%\begin{comment}(BUMP FUNCTION STUFF)
% It can be represented by using a smooth bump function $\rho_k(r)$ that satisfies
%\begin{equation}
%\lim_{r\to \infty } \rho_k(r) = 0, \quad \lim_{r\to 0} \rho_k(r) = -k, \quad \mbox{so that} \quad \int d \rho_k(r) = k.  
%\end{equation}The boundary value of $\rho(r)$ is fixed by the condition 
%\begin{equation}
%\delta_{W_6} = d\rho_k (r) \wedge d \Omega_4^k, \quad \mbox{with} \quad 1 = \int \delta_{W_6} = k \int_{S^4/\mathbb{Z}_k} d \Omega_4^k
%\end{equation} the normalized volume form of $S^4/\mathbb{Z}_k$ is given as
%\begin{equation}
%\frac{8\pi^2}{3} d \Omega_4^k = \frac{1-\mu^2}{4k} d\mu \wedge D\varphi \wedge d \theta \wedge d \psi \sin(\theta) \quad \mbox{with} \quad \int_{S^4/\mathbb{Z}_k} d \Omega_4^k =\frac{1}{k}.
%\end{equation}
%\end{comment}
%
%\paragraph{Symmetry for $k=2$ $(1,0)$ SCFT}
%In general the reduction of M-theory on $S^4/\mathbb{Z}_k$ leads to an $SU(2)_\psi \times SU(k)_\mathrm N \times SU(k)_\mathrm S \times U(1)_\varphi $ gauge symmetry.  This gauge symmetry induces an $SU(2)_\mathcal{R}$ R-symmetry and $SU(k)_\mathrm N  \times SU(k)_\mathrm S  \times U(1)_\varphi $ flavor symmetry on the world volume of the branes.  The $U(1)_\varphi$ symmetry enhances to an $SU(2)_\varphi$ flavor symmetry when $k=2$.  The worldvolume theory on the branes preserve $(1,0)$ symmetry.  
%
%The symmetries can be gauged in the M-theory background by adding gauge field valued on the worldvolume directions of the branes.  From the point of view of the field theory, this corresponds to turning on background gauge fields for the global symmetry.  The boundary condition of $G_4$ flux must be gauge invariant and closed in presence of the gauge fields.  
%We thus have to replace $\overline G_4$ in \eqref{barG4_6d}
%with a 4-form $E_4$ which is closed, gauge-invariant,
%and reduces to $\overline G_4$ when all external
%connections are turned off.
%
%
%
%
%\newpage
%
%
%The 4-form $E_4$ has the following form,
%\beq \label{compact_E4_6d}
%E_4  = 2 \, N \, e_4^{SO(5) \rightarrow SU(2)_\varphi \times SU(2)_\psi}
%+ \frac{F^\mathrm N}{2\pi} \, \omega_{\mathrm N}
%+ \frac{F^\mathrm S}{2\pi} \, \omega_{\mathrm S} \ .
%\eeq
%Our notation is as follows.
%The quantity $e_4^{SO(5)}$ is the global angular form
%on $S^4$, \emph{i.e.}~the closed, gauge-invariant completion
%of the volume form on $S^4$ coupled to arbitrary background
%$SO(5)$ connections.
%The definition and properties of $e_4^{SO(5)}$ are reviewed
%for instance in \cite{sdsd}.
%In the present setup, the action of $\mathbb Z_2$
%breaks the $SO(5)$ isometry  of $S^4$ 
%to the isometry group $SU(2)_\varphi \times SU(2)_\psi$
%of $S^4/\mathbb Z_2$.
%Accordingly, inside $e_4^{SO(5)}$ we only turn on background
%connections along the generators of the 
%$SU(2)_\varphi \times SU(2)_\psi$ subgroup of 
% $SO(5)$.
%Before we consider the action of $\mathbb Z_2$,
%the 4-form $e_4^{SO(5)}$ integrates to 1 on $S^4$.
%After the quotient, $\int_{S^4/\mathbb Z_2} e_4^{SO(5)} = 1/2$,
%which explains the prefactor 2 in \eqref{compact_E4_6d}.
%The 2-forms $F^{\mathrm N, \mathrm S}$ are the field strength
%of the connections associated to the Cartan of the flavor
%symmetry $SU(2)_\mathrm N \times SU(2)_\mathrm S$
%associated to the harmonic 2-forms $\omega_\mathrm N$,
%$\omega_\mathrm S$, as discussed earlier.
%
%
%In order to gauge the $SU(2)_\varphi$ isometry of $S^2_\varphi$
%we find it convenient to introduce three constrained
%coordinates $z^a$, $a = 1,2,3$, satisfying $z^a \, z_a = 1$
%and given by
%\beq
%z^1 = \sin \theta \, \cos \varphi \ , \qquad
%z^2 = \sin \theta \, \sin \varphi \ , \qquad
%z^3 = \cos \theta \ .
%\eeq
%The gauging of $SU(2)_\varphi$ is then performed by introducing the 
%1-forms
%\beq
%Dz^a = dz^a + \epsilon^{abc} \, A_b \, z_c \ ,
%\eeq
%where $A^a$ is the $SU(2)_\varphi$ connection.
%We use the symbol $\widetilde V_2^\varphi$ for the gauged
%version of the volume form on $S^2_\varphi$,
%\beq
%\widetilde V_2^\varphi = \frac{1}{8\pi} \, \epsilon_{abc} \, Dz^a \, Dz^b \, z^c \ .
%\eeq
%This 2-form is not closed, but it admits a closed and gauge-invariant completion,
%which is the global angular form of $SO(3)$ and reads
%\beq
%e_2^\varphi = \widetilde V_2^\varphi  
%- \frac 12 \, \frac{F^a \, z_a}{2\pi} \ ,
%\eeq
%where $F^a$ is the field strength of $A^a$.
%The gauging of $U(1)_\psi$ is performed by replacing $D\psi$
%with $\widetilde D\psi$, which satisfies
%\beq
%d \frac{\widetilde D\psi}{2\pi} = - 2 \, \bigg[ e_2^\varphi + \frac{F^\psi}{2\pi} \bigg] \ .
%\eeq
%The 2-form $F^\psi$ is the curvature
%of the $U(1)_\psi$ external connection $A^\psi$.
%
%After these preliminaries, we can write the 4-form $E_4$.
%It reads
%\begin{align} \label{full_E4_6d}
%E_4 & = \frac 34 \, (1-\mu^2) \, d\mu \, \frac{\widetilde D\psi}{2\pi} \, \widetilde V_2^\varphi
%- \frac 12 \, \mu \, (1-\mu^2) \, \frac{F^\psi}{2\pi} \, \widetilde V_2^\varphi
%- \frac 12 \, \mu \, \frac{\widetilde D\psi}{2\pi} \, \frac{F^\psi}{2\pi}
%\nn \\
%& + \frac 18 \,\mu \, (1-\mu^2) \, \frac{F^a \, Dz_a}{2\pi} \, \frac{\widetilde D\psi}{2\pi}
%+ \frac 14 \, \mu \, (1-\mu^2) \, \widetilde V_2^\varphi \, \frac{F^a \, z_a}{2\pi}
%\nn \\
%& + \frac{\epsilon_{abc} \, z^a \, Dz^b \, F^c}{16 \pi^2} \, d\mu
%- \frac 14 \, d\mu \, \frac{\widetilde D\psi}{2\pi} \, \frac{F^a \, z_a}{2\pi}
%+ \mu \, \bigg[ \frac{F^\psi}{2\pi}\bigg]^2
%- \frac 14 \, \mu \, \frac{F^a \, F_a}{(2\pi)^2}
%\nn \\
%& 
%+ \frac{F^\mathrm N}{2\pi} \, \omega_{\mathrm N}
%+ \frac{F^\mathrm S}{2\pi} \, \omega_{\mathrm S} \ .
%\end{align}
%For definiteness,
%we have written the result for the 
%metric \eqref{sphere2} on $S^2/\mathbb Z_2$,
%for which 
%the function $\gamma(\mu)$ in \eqref{barG4_6d}
%satisfies $\gamma'(\mu) = \frac 34 \, (1-\mu^2)$.
%
%Some comments on \eqref{full_E4_6d}
%are in order. The first term is the gauged version of $\overline G_4$
%in \eqref{barG4_6d}. All other terms with $F^\psi$ and $F^a$ factors
%are needed to ensure that $E_4$ is closed and globally
%well-defined on $S^2/\mathbb Z_2$.
%
%with
%\beq
%d \frac{\widetilde D\psi}{2\pi} = -2 \, e_2^\varphi - 2 \, \frac{F^\psi}{2\pi}
%\eeq 
%and the same conventions for $e_2^\varphi$ as in the appendix of the holography paper.
%
%
%
%
%
%
%
%\begin{align}
%\overline {G}_4 \, \to \, E_4 &=N \left[ d\gamma \wedge \frac{\widetilde{D} \psi}{2\pi} -2 \gamma\left(\frac{F^\psi}{2\pi} + e_2  \right)\right] \wedge e_2 + F^N \omega_N + F^S \omega_S. \label{E46d}
%\end{align} In the gauging, we have turned on the fluctuations of the $C_3$ potentials along the two-cycles, their field strength are $(F^N = d A^N, F^S = dA^S)$.  The gauging of the isometries of $M_4$ is as follows:
%\begin{equation}
%D\psi \, \to \, \widetilde{D} \psi = d \psi + V^\varphi - 2A^\psi, \quad F^\psi = d A^\psi,  \quad dV^\varphi = -2 e_2 \label{6dgauging}
%\end{equation} whereas, $e_2$ is the gauged and closed volume form of the two-sphere $S^2_\varphi$ which can be given in terms of embedding coordinates for the sphere in $\mathbb{R}^3$\footnote{\begin{equation} y^1 = \sin{\theta} \cos(\varphi), \quad y^2 = \sin(\theta) \sin(\varphi), \quad y^3 = \cos(\theta). \end{equation}}.  We have
%\begin{equation}
%4\pi e_2 = \frac{1}{2} \epsilon_{abc} Dy^a \wedge Dy^b y^c + \frac{1}{2} F^{ab} y^c, \qquad Dy^a = dy^a + A^{ab} y^b, \quad F^{ab} = D A^{ab}, \label{spheregin}
%\end{equation} where the gauging is obtained by adding an $SO(3)$ connection, $A^{ab}$, with field strength $F^{ab}$.  The first term in \eqref{E46d} corresponds to the gauging the volume form of the sphere.  The curvature terms are added in order to satisfy the closure condition.  
%



\section{Four-dimensional setup} \label{4dsection}

In this section we describe aspects of the geometric setup when a stack of $N$ M5-branes wrapping a genus, $g$, Riemann Surface $\Sigma_{g,n}$ with $n$ punctures, probe a $\mathbb{C}^2/\mathbb{Z}_2$ singularity in M-theory.  We will discuss various aspects of the geometric setup in M-theory and the symmetries they induce for the field theory that describe the low-energy dynamics of the branes.  We will then use the geometric set-up and compute the anomaly polynomial of the field theory by using anomaly inflow techniques developed in \cite{toappear}.


\subsection{Geometric setup for 4d systems}  

 We consider an eleven-dimensional background given as
\begin{equation} \label{11d_background}
M_{11}  = W^4 \times \Sigma_{g,n} \times \mathbb{C}^2/\mathbb{Z}_2 \times \mathbb{R}.
\end{equation}  
The M-theory background preserves supersymmetry when the space $\Sigma_{g,n} \times \mathbb{C}^2/\mathbb{Z}_2$ satisfies the Calabi-Yau threefold condition, i.e. the first Chern class of the space must vanish.  The worldvolume of the branes decompose as $W^6 = W^4 \times \Sigma_{g,n}$ where $W^4$ is the external spacetime.  The low-energy dynamics of the branes is captured by a field theory that live on $W^4$.  In the region near the branes, the spacetime decomposes as
\begin{equation} \label{near_the_branes}
M_{11} = \mathbb{R}^+ \times M_{10}, \quad \mbox{where} \quad M_6 \hookrightarrow M_{10} \rightarrow W^4, \quad M_4 \hookrightarrow M_6 \rightarrow \Sigma_{g,n}.  
\end{equation} The line $\mathbb{R}^+$ is the overall radius of the transverse directions of the worldvolume spacetime $W^4$.  The space $M_{10}$ describes the tubular neighborhood of the branes, it also corresponds to an internal boundary of the M-theory spacetime near the branes.  Finally, $M_4$ is the resolution space of $S^4/\mathbb{Z}_2$ describe in section \ref{k2res}.  

The Calabi-Yau condition on the M-theory background is satisfied by twisting the R-symmetry circle $S^1_\psi$ over the Riemann surface.  This twist breaks the six-dimensional $SU(2)_\mathcal{R}$ R-symmetry to a $U(1)_\mathcal{R}$ symmetry for the worldvolume theory on $W^4$.  At the level of the geometry, this is achieved by shifting the connection of $S^1_\psi$ as
\begin{equation} \label{hatDpsi}
D\psi \; \to \; \widehat{D} \psi = d\psi + \cos \theta \,  d\varphi -2\pi \, \chi \,  A_\Sigma \ ,
 \quad \mbox{with} \quad  \int_{\Sigma_{g,n}}  dA_\Sigma = 1 \ , \quad \chi  = -2(g-1) - n \ .  
\end{equation} The Euler characteristic of the Riemann surface is denoted by $\chi$.  The twisting, $A_\Sigma$, is a nontrivial component of the six-dimensional gauging of the R-symmetry, $S^\psi$, in \eqref{6dgauging}.  

In addition to twisting the R-symmetry, a large family of four-dimensional SCFTs can be engineered by turn on background fields along the Riemann surface for the Cartan elements of the $SU(2)_\mathrm N \times SU(2)_\mathrm S \times SU(2)_\varphi$ flavor symmetry. Such background fields break the flavor symmetry of the six-dimensional theory to $U(1)_\mathrm N \times U(1)_\mathrm S \times U(1)_\varphi$ for the four-dimensional theory.  At the level of the M-theory background, this is achieved by turning on the following flux parameters
\begin{align}
d\varphi \to \widehat{D} \varphi &= d\varphi +2\pi \,  z \,  A_\Sigma \\
C_3 \to \widehat{C}_3 &= C_3 + 2\pi \, (N_\mathrm N  \, A_\Sigma \wedge \omega_\mathrm N 
+ N_\mathrm S \,  A_\Sigma \wedge \omega_\mathrm S ) \ . \label{fluxgauge}
\end{align}  The connection forms $(N_\mathrm N \,  A_\Sigma, N_\mathrm S\,  A_\Sigma)$ are background fields for the $U(1)$ gauge fields discussed in \eqref{C36d} in the case of $k=2$.  The two-forms $(\omega_\mathrm N, \omega_\mathrm S)$
are the closed representatives that measure the volumes of the resolution two-cycles $(\mathcal{S}_\mathrm N^2, \mathcal{S}_\mathrm S^2)$ in $M_4$.  For every choice of a Riemann surface, $\Sigma_{g,n}$, there is a family of four-dimensional systems labeled by the three flux parameters $(z, N_\mathrm N, N_\mathrm S)$ and the number of branes, $N$.  

 In this paper, we restrict to four-dimensional theories that preserve the $SU(2)_\varphi$ symmetry, this corresponds to fixing $z=0$.  We will also restricted to cases with no punctures, i.e. $n=0$, and non-vanishing  curvature, $g\neq 0$.  For this family, a local metric for $M_6$ can be written as
\begin{equation}
ds^2(M_6) = h_0(\mu) ds^2(\Sigma_g) +  h_1(\mu) ds^2(S^2_\varphi) + h_2(\mu) d\mu^2 +  h_3(\mu) \widehat{D}\psi^2.  \label{M6met}
\end{equation} The interval $\mu$ takes value in $[\mu_\mathrm S, \mu_\mathrm N ]$ where the endpoints are fixed by the loci where $h_3$ vanish.  The functions $(h_0,h_1)$ parametrize the radii of $\Sigma_g$ and $S^2_\varphi$ in $M_6$, they are non-vanishing on the interval of $\mu$.

At a fixed point on the surface $\Sigma_g$, there is a fiber that is a copy of $M_4$ composed of $S^2_\varphi$, the circle $S^1_\psi$ and the interval $\mu$.  Similarly, we can consider a fixed point on the sphere $S^2_\psi$, there are four-dimensional fibers which are copies of a space $M_4^\Sigma$ which are composed of the Riemann surface $\Sigma_g$, the circle $S^1_\psi$ and the interval $\mu$.  These fibers do not shrink in $M_6$.  

\subsection{Flux quantization and four-cycles of $M_6$}  

One of the main object of interest is the boundary condition for the four-flux $G_4$ when the branes wrap the Riemann surface. 
Following \cite{sdsds},
we can write the boundary term for $G_4$ by using a bump function  $\rho(r)$ as
\begin{equation}
G_4 = 2\pi \rho(r) \,  \overline {G}_4 + \dots, \qquad \mbox{with} \qquad \int_{M_4} \overline {G}_4 = N  \ .
\end{equation} The flux $\overline {G}_4$ supports the non-trivial geometry $M_6$.  

The space $M_4$ is the fiber over the Riemann Surface, $\Sigma_g$.  Since it is non-shrinking, we can thread $N$ units of flux on it at a fixed point of the Riemann surface.  Similarly, at a fixed point of the sphere, $S^2_\varphi$, we can thread flux on the fiber $M_4^\Sigma$ given as 
\begin{equation}
\int_{M_4} \overline {G}_4 = N_\Sigma.  
\end{equation}  The space $M_6$ also admits four-cycles localized at the north and south poles of the $\mu$ interval where $S^1_\psi$ shrinks.  These correspond to the product of the resolution cycles of the original orbifold singularities of the $S^4/\mathcal{Z}_2$ with the Riemann surface, $\Sigma_g$.  They are denoted as
\begin{align}
\mathcal{C}_\mathrm N^4 &= \mathcal{S}^2_\mathrm N \times \Sigma_g & &   
\hspace{-3cm} \mbox{localized at} \qquad \mu = \mu_\mathrm N \ , \\
\mathcal{C}_\mathrm S^4 &= \mathcal{S}^2_\mathrm S \times \Sigma_g & &\hspace{-3cm}  \mbox{localized at} \qquad \mu = \mu_\mathrm S \ .
\end{align} We can thread flux on these cycles given as 
 \begin{equation} \label{N_north_south_def}
 \int_{\mathcal{C}_\mathrm N^4} \overline {G}_4 = N_\mathrm N \in \mathbb{Z}, \qquad  \int_{\mathcal{C}_\mathrm S^4} \overline {G}_4 = N_\mathrm S \in \mathbb{Z}.
\end{equation} It seems then that there exist four flux quanta $(N,N_\Sigma,N_\mathrm N,N_\mathrm S)$ that label the class of $\overline {G}_4$ in $M_6$.  These flux parameters are not all independent.  This reflects the fact that the space $M_6$ actually admits only three four-cycles denoted as $(\mathcal{C}_\mathrm N^4, \mathcal{C}_\mathrm S^4,  \mathcal{C}_\mathrm C^4)$.  The last one $\mathcal{C}_\mathrm C^4$ is not localized on $M_6$.  

To see that there are only three independent flux parameters, we consider the most general local expression for $\overline {G}_4$ that is closed and consistent with the symmetries of $M_6$
%\begin{equation}
%8\pi^2 \bar{G}_4 = d\gamma_\varphi(\mu) \wedge  \hat{D} \psi \wedge d\Omega_2^\varphi + d \gamma_\Sigma(\mu) \wedge \hat{D} \psi \wedge d\Sigma_g - \left(\gamma_\varphi + \gamma_\Sigma \right) d\Sigma_g \wedge d\Omega_2^\varphi  
%\end{equation}
\begin{equation} \label{overlineG4_4d}
\overline G_4= d\gamma_\varphi(\mu) \wedge  \frac{\widehat{D} \psi}{2\pi} \wedge 
V_2^\varphi
+ d \gamma_\Sigma(\mu) \wedge \frac{\widehat{D} \psi}{2\pi} \wedge  V^\Sigma_2 
- 2 \,  \left(\gamma_\varphi + \gamma_\Sigma \right)  V^\Sigma_2  \wedge 
V_2^\varphi   \ ,
\end{equation}
where $V^\varphi_2$, $V^\Sigma_2$ are proportional to the volume forms of $S^2_\varphi$ and the Riemann surface, respectively, normalized
according to
\beq \label{Vnormalization}
\int_{S^2_\varphi} V_2^{\varphi} = 1 \ , \qquad
\int_{\Sigma_g} V^\Sigma_2 = \frac \chi 2  \ .
\eeq
  The flux parameters are given as
\begin{equation} \label{gamma_eqs}
\gamma_\varphi^\mathrm N - \gamma_\varphi^\mathrm S = N \ , \quad \left(\gamma_\Sigma^\mathrm N - \gamma_\Sigma^\mathrm S \right) \chi = 2 N_\Sigma \ , \quad \left(\gamma^\mathrm N_\varphi + \gamma^\mathrm N_\Sigma \right) \chi 
=-N_\mathrm N \ , \quad \left(\gamma^\mathrm S_\varphi + \gamma^\mathrm S_\Sigma \right) \chi = -N_\mathrm S \ ,
\end{equation} where the $\gamma$ parameters are defined as $\gamma_{\bullet}^{N/S} \equiv \gamma_{\bullet}(\mu_{N/S})$.  The $\gamma$ relations imply\footnote{The constraint on the flux parameters can be understood as the condition that must be satisfied by the first Chern class of the $S^1_\psi$ bundle over the rest of the space:
\begin{equation}
\int_{\mathcal{C}_\mathrm N^4} \overline {G}_4 - \int_{\mathcal{C}_\mathrm S^4} \overline {G}_4 = \int_{M_6} \overline {G}_4\, d\frac{\widehat{D} \psi}{2\pi}.  
\end{equation} The minus sign is due the fact that the two cycles have opposite orientations in $M_6$.  }
\begin{equation}
2N_\Sigma + \chi N = - (N_\mathrm N - N_\mathrm S) \ .  
\end{equation}  The class $G_4$ is labeled by three flux parameters that we denote as $(N,N_\mathrm N, N_\mathrm S)$.  The flux parameter $N$ can be associated with the four-cycle $\mathcal{C}_\mathrm C^4$.

Another way to interpret the fluxes $(N_\mathrm N,N_\mathrm S)$ is to consider the fate of the fluctuations of the $C_3$ potential from the $SU(2)_\mathrm N\times SU(2)_\mathrm S$ symmetry before the compactification on the Riemann surface.   The curvatures associated to $SU(2)_\mathrm N\times SU(2)_\mathrm S$
are   $(F_{6d}^\mathrm N,F_{6d}^\mathrm S)$. 
We use the notation $(F_\text{$6d$, Cartan}^\mathrm N,F_\text{$6d$, Cartan}^\mathrm S)$
for the curvatures of the Cartan subgroup  $U(1)_\mathrm N\times U(1)_\mathrm S$.
 Since these forms have legs on the worldvolume directions of the M5-branes, $W_6$, when we compactify on the Riemann surface, they decompose as
%\begin{equation}
%F^{N} = N_N d\Sigma_g + F^N_{4d}, \quad F^{S} = N_S d\Sigma_g + F^S_{4d}.  
%\end{equation}
\begin{equation} \label{fluxes_6d_to_4d}
\frac{F_\text{$6d$, Cartan}^{\mathrm N}}{2\pi} = N_\mathrm N \,  (2 \, \chi^{-1 } \,  V_2^\Sigma)    + 
N \, \frac{F^\mathrm N }{2\pi}, \qquad 
\frac{F_\text{$6d$, Cartan}^{\mathrm S}}{2\pi} = N_\mathrm S  \,  (2 \, \chi^{-1 } \,  V_2^\Sigma) 
+ N \,  \frac{F^\mathrm S }{2\pi} \ .  
\end{equation}
The quantities $(F^\mathrm N, F^\mathrm S)$ are 4d external
connections. We have introduced a factor $N$ in such a way that
both terms on the RHSs of \eqref{fluxes_6d_to_4d} scale linearly with the flux parameters $N$, $N^\mathrm N$, $N^\mathrm S$.
In the reduction, this decomposition implies the flux terms in $\overline {G}_4$ as 
%\begin{equation}
%\bar{G}_4 = N_N d\Sigma_g \wedge \omega_N + N_S d\Sigma_g \wedge \omega_S + \dots
%\end{equation}
\begin{equation}
\overline {G}_4 = N_\mathrm N  \,  (2 \, \chi^{-1 } \,  V_2^\Sigma) \wedge \omega_\mathrm N +
 N_\mathrm S  \,  (2 \, \chi^{-1 } \,  V_2^\Sigma) \wedge \omega_\mathrm S + \dots
\end{equation}
In field theory, the flux correspond to twisting the Cartan elements of the six-dimensional $SU(2)_\mathrm N \times SU(2)_\mathrm S$ symmetry over the Riemann surface.  

There are three harmonic two-forms associated to the four-cycles by Poincar\'{e} duality, we denote them as $(\omega_\mathrm N, \omega_\mathrm S, \omega_\mathrm C)$.  Indeed, the first two are just the resolution two cycles of $M_4$ which are preserved in $M_6$.  The flux quantization conditions can be equivalently written as
\begin{equation} \label{poincare_duality}
\int_{M_6} \overline {G}_4 \wedge \omega_\mathrm N = N_\mathrm N, \qquad \int_{M_6} \overline {G}_4 \wedge \omega_\mathrm S = N_\mathrm S, \qquad \int_{M_6} \overline {G}_4 \wedge \omega_\mathrm C = N.  
\end{equation} These formulas will be useful in the computation of the anomalies for the four-dimensional theories of interest.  


In the reduction of M-theory on $M_6$, there are a class of fluctuations we can add for the $C_3$ potential.  For each of the harmonic two-forms, we can add a gauge field in the external spacetime given as $(a^\mathrm N, a^\mathrm S, a^\mathrm C)$ with field strength $(f^\mathrm N, f^\mathrm S, f^\mathrm C)$.  
We are using lowercase letters to emphasize that these are
gauge fields in 7d supergravity.
Naively, each one of these fields should lead to a $U(1)$ gauge symmetry on the external spacetime which then induces a $U(1)$ flavor symmetry on the worldvolume theory on the branes.  However, the $C_3$ potential can also have a three-form fluctuation, $c_3$, on the external spacetime with field strength, $g_4 = dc_3$.  These terms can be collected as
\begin{equation}
C_3 = a^\mathrm N \wedge \omega_\mathrm N + a^\mathrm S \wedge \omega_\mathrm S + a^\mathrm C \wedge \omega_\mathrm C + c_3+ \dots  
\end{equation} When we reduce the effective action of M-theory, the effective action of the seven-dimensional theory will have terms
\begin{equation} \label{7d_action}
S = \int  b_1 g_4 \wedge \star g_4 + b_2 N_\alpha a^\alpha \wedge g_4 + \dots
\end{equation} where the $b$'s are numbers.  We observe that $g_4$ couples to a linear combination of the gauge field.  This coupling implies that $g_4$ can be dualized to a St\"uckelberg field which is eaten by the gauge field $N_\alpha a^{\alpha}$.  Here and in what follows, the index $\alpha$ enumerates harmonic 2-forms
and takes the values $\alpha = \mathrm N, \mathrm S, \mathrm C$.
We refer the reader to \cite{toappear} for a more detailed
discussion of this St\"uckelberg mechanism.

In holography: \cite{Gubser:2008px, Hartnoll:2008vx}


\paragraph{Symmetries of the system}  The low-energy quantum field preserves a $U(1)_\mathcal{R}$ R-symmetry and the $SU(2)_\varphi$ flavor symmetries corresponding to the isometries of $S^1_\psi$ and $S^2_\varphi$.  Naively there is an $U(1)_\mathrm N \times U(1)_\mathrm  S \times U(1)_\mathrm  C$ corresponding to the fluctuations of $C_3$ along the harmonic two-forms $(\omega_\mathrm  N, \omega_\mathrm  S, \omega_\mathrm  C)$.  One linear combination is broken and only a $U(1)^2$ is preserved, which we denote as $U(1)_\mathrm  N \times U(1)_\mathrm  S$.  In the special cases when $g=0$, the Riemann surface is a two-sphere, in the low-energy limit it can admit an $SU(2)$ isometry group.  The flavor symmetry will further enhance by an $SU(2)$ flavor symmetry.  

Now we are in a position to construct the gauge invariant and globally defined boundary condition for the $G_4$ flux in presences of curved branes.  We have the action of the symmetries in $\overline {G}_4$ by adding suitable connection forms and curvature terms to make it closed:
%\begin{align}
%2\pi \bar{G}_4 \, \to \, 2\pi E_4 &=  d\left[\gamma_\varphi(\mu) \wedge  \widetilde{D} \psi \wedge e_2^\varphi + d \gamma_\Sigma(\mu) \wedge \widetilde{D} \psi \wedge e_2^\Sigma \right] \\
%&+ F^N \omega_N +  F^S \omega_S + F^C \omega_C, \qquad \mbox{with} \quad  F^\alpha N_\alpha =0.
%\end{align}
\begin{align} \label{final_E4}
\overline {G}_4 \, \to \, E_4 &=  d \bigg[\gamma_\varphi(\mu) \wedge 
\frac{ \widetilde{D} \psi }{2\pi} \wedge e_2^\varphi + \gamma_\Sigma(\mu) \wedge \frac{\widetilde{D} \psi}{2\pi} \wedge e_2^\Sigma \bigg]  \nn \\
&+N \,  \frac{F^\mathrm  N}{2\pi} \wedge  \widetilde \omega_\mathrm  N 
+  N \, \frac{F^\mathrm  S}{2\pi} \wedge \widetilde \omega_\mathrm  S
 + N \,  \frac{F^\mathrm  C}{2\pi} \wedge  \widetilde \omega_\mathrm  C \ , \qquad \mbox{with} \quad  F^\alpha N_\alpha =0 \ .
\end{align}
The last condition imposes the fact that one of gauge fields in the fluctuations of the $C_3$ potential is massive.  In the expression for $E_4$ we have gauged the isometry group as
%\begin{align}
%\widetilde{D} \psi = d \psi + V^\varphi + V^{\chi} - 2 F^\psi_{4d}, \quad F^\psi_{4d} = d A^\psi_{4d},  \quad dV^\varphi = -4\pi e_2^\varphi, \quad d V^\chi = - 4\pi e^\Sigma_2.  
%\end{align}
\begin{align} \label{tildeDpsi}
\frac{\widetilde{D} \psi}{2\pi} = \frac{d \psi}{2\pi}  - 2 \, \bigg( \cA^\varphi + \cA^{\Sigma} -  
 \frac{ A^\psi }{2\pi} \bigg), \qquad   d A^\psi = F^\psi ,  \qquad d \cA^\varphi = e_2^\varphi, \qquad
d \cA^\Sigma =   e^\Sigma_2 \ .  
\end{align}
The quantity $A_\psi$ is the 4d connection for the $U(1)_\psi$ isometry.
The two-forms, $e^\varphi_2$ and $e_2^\Sigma$ are the closed and gauge invariant volume forms of $S^2_\psi$ and $\Sigma_g$ respectively. 
The expression for $e_2^\varphi$~is
\beq \label{e2_def}
e_2^\varphi = \frac{1}{8\pi} \, \epsilon_{abc} \, (Dy^a \wedge Dy^b \, y^c - F^{ab} \, y^c)
\ , \qquad Dy^a = dy^a - A^{ab} \, y_b \ .
\eeq
The indices $a,b,c = 1,2,3$ are vector indices of $SO(3)_\varphi$,
raised and lowered with $\delta_{ab}$. The three quantities $y^a$
are constrained coordinates on $S^2_\varphi$, with $y^a \, y_a = 1$.\footnote{More explicitly,
\beq
y^1 = \sin \theta \, \cos \varphi \ , \qquad
y^2 = \sin \theta \, \sin \varphi \ , \qquad
y^3 = \cos \theta \ .
\eeq
}
The 1-forms $A^{ab}$ are the components of the external $SO(3)_\varphi$ connection,
and $F^{ab}$ are the components of the field strength.
When $g>1$, $e_2^\Sigma$ is simply the volume form on the Riemann surface,
$e_2^\Sigma = V_2^\Sigma$.
When $g = 0$ and the surface is a sphere, $e_2^\Sigma$
is given similarly as \eqref{e2_def}.
We need the integrals
\begin{equation} \label{integral_identities}
\int_{\Sigma_g} e_2^\Sigma = \frac{\chi}{2}, \qquad \int_{S^2} e_2^{2s+2} = 0, \quad \int_{S^2} e_2^{2s+1} = 2^{-2s} \left[p_1(SO(3)) \right]^s, \quad s=0,1,2, \cdots
\end{equation} where $p_1(SO(3)_\varphi)$ is the first Pontryagin class of the $SO(3)_\varphi$ bundle over $W^4$.

The tilde over the harmonic 2-forms $\omega_{\mathrm N, \mathrm S, \mathrm C}$ 
in \eqref{final_E4}
signals the fact that we have gauged the isometry group
and we have restored closure, as explained below.


\paragraph{Harmonic 2-forms}  Before 
gauging the isometry group, the harmonic
2-forms $\omega_\alpha$, $\alpha  = \mathrm N, \mathrm S, \mathrm C$, can be uniformly 
parametrized as
\beq
\omega_\alpha = d \bigg[ H_\alpha(\mu) \, \frac{\widehat D\psi}{2\pi} \bigg]
+ t^\varphi_\alpha  \, V_2^\varphi 
+ t^\Sigma_\alpha \, V^\Sigma_2 \ ,
\eeq
where $t_\alpha^\varphi$, $t_\alpha^\Sigma$ are suitable constants
and $H_\alpha$ is a suitable function of $\mu$.
We promote $\omega_\alpha$ to $\widetilde \omega_\alpha$
by writing
\beq
\widetilde \omega_\alpha = d \bigg[ H_\alpha(\mu) \, \frac{\widetilde  D\psi}{2\pi} \bigg]
+ t^\varphi_\alpha  \, e_2^\varphi 
+ t^\Sigma_\alpha \, e^\Sigma_2 \ .
\eeq
This object is indeed manifestly closed and gauge-invariant.

The choice of basis $\omega_{\mathrm N, \mathrm S, \mathrm C}$ is specified by the relations
\eqref{poincare_duality}.
They imply
\beq \label{H_table}
\begin{array}{l  || c | c | c|cc}
  & \phantom{l} H_\alpha^{\rm N} \phantom{l}  & \phantom{l} H_\alpha^{\rm S}  \phantom{l} & \phantom{l} t_{\alpha}^\varphi \phantom{l} &
  \phantom{l}  t_{\alpha }^\Sigma \phantom{l} \\[1mm]  \hline
\alpha = C \phantom{l}& 0 & 0 & 0 & \frac 2 \chi \\[1mm]
\alpha = N \phantom{l}& \frac 12 & - \frac 12 & -1 & -1 \\[1mm]
\alpha = S \phantom{l}& \frac 12 &  - \frac 12 & 1 & 1 
\end{array}
\eeq
This table summarize all information about $\omega_\alpha$
that is needed for the computation of  anomaly inflow in the next section.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
\paragraph{Two-cycles of $M_6$} The space $M_6$ admit three two-cycles labeled as $(\mathcal{S}^2_N,\mathcal{S}^2_S, \mathcal{S}^2_C)$.  The first two, $(\mathcal{S}^2_N,\mathcal{S}^2_S)$, are inherited from $M_4$ and are localized at the end of the interval of $\mu$ where $S^1_\psi$ shrink.  The two-cycle, $\mathcal{S}^2_C$ is a linear combination of the Riemann surface, $\Sigma_{g}$, and the sphere $S^2_\varphi$.  This two-cycle of $M_6$ is defined by the condition
\begin{equation}
\frac{1}{2\pi} \int_{\mathcal{S}^2_C} d \hat{D} \psi =0, \quad \mbox{it is given as} \quad  \mathcal{S}^2_C = 2 \Sigma_g - \chi S^2_\varphi  .  
\end{equation} 

The low-energy dynamics preserves an additional $U(1)$ symmetry, that is obtained from the fluctuations of $C_3$ along the new two-cycle $S^2_\mathcal{C}$.  We denote the harmonic form representative of volume of the cycle by $\omega^2_C$.  
\end{comment}




\begin{comment}
The global four-forms associated to the four-cycles are $(V_4, V_N = V_\Sigma \times \omega_N, V_S = V_\Sigma \times \omega_S)$ where $V_\Sigma$ is a normalized volume form of the Riemann surface that integrates to $2\pi$, i.e. $V_\Sigma = dA_\Sigma$.  The first form, $V_4$, corresponds to the volume form of the four-sphere, $S^4$.  Integrating the $G_4$ flux on these cycles yield the following quantization conditions
\begin{equation}
\frac{1}{2\pi} \int_{M_4} G_4 = N \in \mathbb{Z}, \quad \frac{1}{2\pi} \int_{\mathcal{C}_N^4} G_4 = N_N \in \mathbb{Z}, \quad \frac{1}{2\pi} \int_{\mathcal{C}_S^4} G_4 = N_S \in \mathbb{Z}.
\end{equation}   The flux parameters for $G_4$ from the localized four-cycles are precisely the same as those from the background field for $U_N(1) \times U_S(1)$ in \eqref{fluxgauge}.  A representative of $V_4$ can be written as
\begin{equation}
V_4 = d\gamma(\mu) \wedge \hat{D} \psi \wedge d\Omega_2^\varphi + \gamma(\mu) d A_\Sigma \wedge d\Omega_2^\varphi.    
\end{equation} The function $\gamma(\mu)$ must vanish at the end points of the $\mu$ interval, it is normalized such that the integral of $V_4$ on the sphere is 1.  It is explicit value is not necessary for the analysis that follows. The class of $G_4$ on $M_6$ can be written as 
\begin{equation}
G_4 = N V_4 + N_N V_\Sigma \wedge \omega_N +  N_S V_\Sigma \wedge \omega_S.   
\end{equation}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Anomalies for the low energy QFT}  


%\begin{comment}(DISCUSSION ABOUT ANOMALY POLYNOMIAL)

Now we are in a position to compute anomalies for M5-branes probing the $k=2$ orbifold singularity.  The construction of the boundary data above will allow for an explicit computation for the anomaly polynomial for the field theories that describe the low energy dynamics of the branes \cite{Bah:2018gwc,Bah:2019jts,toappear}.  These are captured by a 12-form M-theory anomaly polynomial given as
\begin{equation} \label{I12_and_X8}
\mathcal{I}_{12} = - \frac{1}{6} E_4^3 - E_4 \wedge X_8, \qquad X_8 = \frac{1}{192} \left[p_1(TM_{11})^2  - 4\,  p_2(TM_{11}) \right]  \ ,
\end{equation} where $p_1(TM_{11})$, and $p_2(TM_{11})$ are the first and second Pontryagin classes of the tangent bundle of the eleven-dimensional M-theory spacetime, $TM_{11}$.  The four-form $E_4$ is precisely the gauge invariant boundary and globally defined boundary condition for the $G_4$ flux.  The anomaly six-form for the four-dimensional theories discussed above is given as
\begin{equation} \label{I12_integral}
I_6^{\rm inflow} = \int_{M_6} \mathcal{I}_{12}   \ ,
\end{equation} where we use the corresponding $E_4$ given in \eqref{final_E4}.  

%\subsubsection*{Anomalies for 6D theories}
%
%Anomaly inflow for flat M5-branes probing orbifold singularities was studied in \cite{Ohmori:2014kda}.  In the region near the branes, the tangent bundle of M-theory decompose as
%\begin{equation}
%TM_{11} \, \to \, TW_6 \oplus TM_4
%\end{equation} where $W_6$ is the worldvolume directions of the branes.  

%\subsubsection*{Anomalies for 4D theories}

The task at hand is the computation of the 8-form $X_8$
for the geometry \eqref{M6met} and of the integrals
$\int_{M_6} E_4 \, X_8$, $\int_{M_6} E_4^3$
with $E_4$ as in \eqref{final_E4}.
The full derivation is reported in detail in \cite{sdsd}.
Here we point out some salient features of the analysis.


The 8-form $X_8$ is constructed with the first and second
Pontryagin classes of the 11d tangent bundle $TM_{11}$,
see \eqref{I12_and_X8}.
For the class of 4d theories under examination,
these classes can be computed using the following splitting
of $TM_{11}$,
\beq \label{bundle_split}
TM_{11} \rightarrow TW_4 \oplus T\Sigma_{g} \oplus 
TS^2_\varphi \oplus TS^2_{\mu\psi}  \  .
\eeq
The above expression is motivated recalling
that the space $M_6$ is a fibration of
$M_4$ (the resolved orbifold $S^4/\mathbb Z_2$)
over $\Sigma_g$, and that $M_4$
is a fibration of the 2-sphere $S^2_{\mu \psi}$ spanned by
$\mu$, $\psi$ over the 2-sphere $S^2_\varphi$.
The gauging of the isometry $SO(3)_\varphi$
shifts the Chern root of $TS^2_\varphi$
with a contribution with legs along $W_4$.
By a similar token, the Chern root of 
$TS^2_{\mu \psi}$ is shifted by the fact that $S^1_\psi$
is non-trivially fibered over $S^2_\varphi$, $\Sigma_g$,
and $W_4$, as can be inferred from the expression
of $\widetilde D\psi$ in \eqref{tildeDpsi}.
The split \eqref{bundle_split} implies 
\begin{align}
p_1(TM_{11}) & = p_1(TW_4) + p_1(SO(3)_\varphi)
+ \bigg[ d  \frac{\widetilde D\psi}{2\pi} \bigg]^2 \  , \nn \\
p_2(TM_{11}) & = \big[  p_1(TW_4) + p_1(SO(3)_\varphi)
\big] \, \bigg[ d  \frac{\widetilde D\psi}{2\pi} \bigg]^2 \ .
\end{align}
We noticed that 
  terms with more than six external legs,
such as $p_1(TW_4) \,p_1(SO(3)_\varphi)$,
can be dropped, because they cannot
contribute to the the inflow anomaly
polynomial.




 
%Let us now comment on the computation
%of the integrals $\int_{M_6} E_4^3$, $\int_{M_6} E_4 \, X_8$.
%Their values are insensitive to the specific
%profiles of the functions $\gamma_\varphi$,
%$\gamma_\Sigma$, $H_\alpha$
%entering $E_4$,
%and only depend on the values that these functions
%attain at the endpoints of the $\mu$ interval.
%For the functions $H_\alpha$, these values
%are collected in \eqref{H_table}.
%The 
%four quantities $\gamma_{\varphi, \Sigma}^{\rm N,S}$
%we have to 


As pointed out earlier, the background curvatures
for the $U(1)$ symmetries associated to harmonic 2-forms
are subject to the constraint $F^\alpha N_\alpha = 0$.
This is due to the  
 argument given around \eqref{7d_action} for the 
emergence of a massive vector in 7d supergravity.
This argument, however,
 is
valid under the technical assumption 
\beq \label{condition}
\int_{M_6} \overline G_4 \wedge \omega_\psi = 0 \ .
\eeq
In the previous expression $\overline G_4$ is as in \eqref{overlineG4_4d}
and the 2-form $\omega_\psi$ is the coefficient of the linear term in $F^\psi$
inside $E_4$,
\beq
E_4 = F^\psi \wedge \omega_\psi + \dots \ , \qquad
\omega_\psi = 2 \, (2 \pi)^{-1} \, (\gamma_\varphi \, e_2^\varphi
+ \gamma_\Sigma \, e_2^\Sigma) \ .
\eeq
The requirement \eqref{condition}
ensures that the linear combination
of 7d $U(1)$ vectors  that gets massive via
St\"uckelberg mechanism
is built exclusively with the vectors
associated to harmonic 2-forms,
without any mixing with the vector $A^\psi$
associated to the isometry $U(1)_\psi$.
The interested reader can find a more
detailed discussion of this point in 
 \cite{sdsd}.
If we combine \eqref{condition} with the relations
\eqref{gamma_eqs}, we can express the four quantities
$\gamma_\varphi^\mathrm N$, $\gamma_\varphi^\mathrm S$,
$\gamma_\Sigma^\mathrm N$, $\gamma_\Sigma^\mathrm S$
in terms of the three flux quanta
$(N, N_\mathrm N, N_\mathrm S)$,
\begin{align} \label{gamma_endpoints}
\gamma_\varphi^{\rm N,S} &= - \frac{N \, (N_\mathrm N + N_\mathrm S)}{ 2 \, (2 \chi N  + N_\mathrm N - N_\mathrm S )} \pm \frac 12 \, N \ , \\
\gamma_\Sigma^{\rm N,S} &=
- \frac{(N_\mathrm N + N_\mathrm S) (\chi N + N_\mathrm N - N_\mathrm S)}{2 \chi \, (
2 \chi N + N_\mathrm N - N_\mathrm S
)} 
\mp \frac 14 (\chi N  + N_\mathrm N - N_\mathrm S)  \ .
\end{align}

It is worth noticing that the values of the integrals $\int_{M_6} E_4 \, X_8$,
$\int_{M_6} E_4^3$ are insensitive to the specific profile of the functions
$\gamma_\varphi$, $\gamma_\Sigma$, $H_\alpha$ entering $E_4$, but only depend on the values
that these functions attain at the endpoints of the $\mu$ interval.
For $\gamma_\varphi$ and $\gamma_\Sigma$
these values are given in \eqref{gamma_endpoints},
while for $H_\alpha$ they are collected in \eqref{H_table}.
We also notice that integration over $S^2_\varphi$ of powers of $e_2^\varphi$
 is conveniently
preformed making use of \eqref{integral_identities},
and similarly for integration along the Riemann surface.


After these preliminary remarks, we can give the full
expression for the inflow anomaly polynomial
$I_6^{\rm inflow}$ computed via \eqref{I12_integral}.
It reads
\begin{align} \label{total_inflow}
- I_6^{\rm inflow}
& =
 \bigg[ 
-\frac{2 \,  N^2 \,  \left( \chi   N    +N_{\rm N} \right) \left(   
   \chi   N - N_{\rm S} \right) \left(  \chi   N
   +N_{\rm N} - N_{\rm S}  \right)}{\left(2 \chi N  
   +N_{\rm N} - N_{\rm S} \right){}^2}
 +  \frac \chi 2 \, N
\bigg] \, \bigg[  \frac{ F^\psi}{2 \pi} \bigg] ^2 \, 
\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
\nn \\
& + \frac{2  \, N^2 \,   N_{\rm N}  \left(N_{\rm N} + \chi N
   \right) }{2 \chi N
   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi}{2\pi} \, \frac{F^\mathrm N}{2\pi} \, \bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
   + \frac{2  \, N^2 \,   N_{\rm S}
   \left(N_{\rm S} - \chi N \right) }{2 \chi N
   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi }{2\pi} \, \frac{ F^\mathrm S }{2\pi} \, 
\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
\nn \\
& + \bigg(  N^2 \, N_\mathrm N   + \frac 23  \chi N^3 \bigg) \,  \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^3
+ \bigg( -  N^2 \, N_\mathrm S   + \frac 23  \chi N^3 \bigg) \, 
 \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^3
 \nn \\
& + N^2 \, N_\mathrm S \, \frac{ F^{\rm S} }{2\pi} \, 
 \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^2
- N^2 \, N_\mathrm N    \, \frac{ F^{\rm N} }{2\pi} \, 
 \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^2
 + \frac 16 \,  (N_{\rm N} - N_{\rm S})  \, \bigg[  \frac{ F^\psi}{2 \pi} \bigg] ^3
\nn \\
&  - \frac{1}{24} \, (N_{\rm N} - N_{\rm S}) \, \frac{F^\psi }{2\pi} \, p_1(TW_4)
- \frac{\chi}{24} \,\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg) \, p_1(TW_4)
\nn \\
&  + \bigg[
\frac{N^2 \left(\chi^2 N^2 
-3 \,
   N_{\rm N} N_{\rm S}+2 \,  \chi N ( N_{\rm N}  - N_{\rm S}) \right)}{6
   \left(2 \chi N +N_{\rm N} - N_{\rm S}\right)}
   - \frac{\chi}{12} \, N
   \bigg] \, \frac{F^\psi }{2\pi}\, p_1(SO(3)_\varphi)
   \nn \\
& - \frac 14 \, N^2 \, \bigg(N_{\rm N} \, \frac{F^{\rm N}  }{2\pi}
- N_{\rm S} \, \frac{ F^{\rm S} }{2\pi} \bigg)   \, p_1(SO(3)_\varphi)   \ .
\end{align}
%\begin{align} \label{total_inflow}
%- (2\pi)^3 \, I_6^{\rm inflow}
%& =
%\frac 16 \,  (N_{\rm N} - N_{\rm S})  \, (F^\psi)^3
%\nn \\
%&+ \bigg[ 
%-\frac{2 \,  N \,  \left(N   \chi +N_{\rm N} \right) \left(N  
%   \chi - N_{\rm S} \right) \left(\chi N
%   +N_{\rm N} - N_{\rm S}  \right)}{\left(2 N \chi
%   +N_{\rm N} - N_{\rm S} \right){}^2}
% +  \frac \chi 2
%\bigg] \, (F^\psi)^2 \, ( F^{\rm N}  + F^{\rm S} )
%\nn \\
%& + \frac{2  \left(F^{\rm S} N_{\rm S}
%   \left(N_{\rm S} - N \chi \right)+F^{\rm N} N_{\rm N}  \left(N_{\rm N} + N \chi
%   \right)\right)}{2 N \chi
%   +N_{\rm N} - N_{\rm S}} \, F^\psi \, \left(F^{\rm N}+F^{\rm S}\right)
%\nn \\
%& + \bigg(  \frac{N_{\rm N}}{N} + \frac 23  \chi \bigg) \, (F^{\rm N})^3
%+ \bigg( - \frac{N_{\rm S}}{N} + \frac 23  \chi \bigg) \, (F^{\rm S})^3
%+ \frac{N_{\rm S}}{N} \, F^{\rm S} \, (F^{\rm N})^2
%- \frac{N_{\rm N}}{N} \, F^{\rm N} \, (F^{\rm S})^2
%\nn \\
%&  - \frac{1}{24} \, (N_{\rm N} - N_{\rm S}) \, F^\psi \, p_1(TW_4)
%- \frac{\chi}{24} \, (F^{\rm N} + F^{\rm S}) \, p_1(TW_4)
%\nn \\
%&  + \bigg[
%\frac{N^2 \left(N^2 \chi ^2
%-3 \,
%   N_{\rm N} N_{\rm S}+2 \,  N \chi ( N_{\rm N}  - N_{\rm S}) \right)}{6
%   \left(2 N \chi +N_{\rm N} - N_{\rm S}\right)}
%   - \frac{\chi}{12} \, N
%   \bigg] \, F^\psi \, p_1(SO(3)_\varphi)
%   \nn \\
%& - \frac 14 \, N \, (N_{\rm N} \, F^{\rm N} - N_{\rm S} \, F^{\rm S})   \, p_1(SO(3)_\varphi)   \ .
%\end{align}
We have solved the constraint $F^\alpha N_\alpha = 0$
by expressing $F^\mathrm C$ in \eqref{final_E4} in terms of $F^{\rm N,S}$,
\beq
F^\mathrm C = - \frac 1N \, (N_\mathrm N \, F^\mathrm N
+ N_\mathrm S \, F^\mathrm S) \ .
\eeq


 

\section{Holographic solutions}  

In the previous sections we have adopted a UV
point of view:  we fixed the supersymmetric M-theory
background \eqref{11d_background}
and we inserted a stack of M5-branes 
extended along $W_4 \times \Sigma_g$
and sitting at the origin of $\mathbb C^2/\mathbb Z_2 \times \mathbb R$, specifying also the appropriate
background fluxes along the Riemann surface.
In this section we argue that, in the large-$N$ limit,
this class of UV setups corresponds in the IR 
to a well-known class of $AdS_5$ solutions
in M-theory, first described in GMSW \cite{Gauntlett:2004zh}.


In the vicinity of the M5-branes,
the UV picture of 11d spacetime 
is described in \eqref{near_the_branes}.
Our expectation for the near-horizon IR picture, based on \cite{gauntlett_flows},
is that the overall radial direction $\mathbb R^+$
combines with $W_4$ to yield
an $AdS_5$ factor, leaving the geometry $M_6$
as internal space. Taking into account backreaction
effects, the Ansatz for the 11d metric in the near-horizon limit has the form
\beq
ds^2(M_{11}) = e^{2\lambda} \, \big[ ds^2(AdS_5)
+ ds^2(M_6) \big] \ ,
\eeq
with $ds^2(M_6)$ of the form \eqref{M6met},
and $\lambda$ a warp factor depending on $M_6$.
Let us stress that all metric functions
in the ansatz \eqref{M6met} for the metric on $M_6$
depend on the interval coordinate $\mu$ only.
It is natural to also demand that
the warp factor $\lambda$ be a function of $\mu$ only.

In \cite{Gauntlett:2004zh} a class of solutions is described,
in which $M_6$ and $\lambda$ have exactly 
the properties described in the previous paragraph.
More precisely, the fully backreacted geometry of $M_6$ is
\beq \label{IRgeometry}
ds^2(M_6)  = e^{-6\lambda} \Big[ F_{\varphi} \, d  s^2(S^2_\varphi)
+ F_\Sigma \, d  s^2(\Sigma_g) \Big]
+ \frac{e^{-6\lambda}}{\cos^2\zeta} d\mu^2
+ \frac{\cos^2 \zeta}{9} \widehat D\psi^2 \ ,
\eeq
where the warp factor $\lambda$ and the metric functions
$F_\varphi$, $F_\Sigma$, $\cos \zeta$ depend on $\mu$ only.
Their expressions are recorded in appendix \ref{sugra_app},
where we summarize some key features of the GMSW solutions. 
The $G_4$-flux configuration of the holographic solution
is given in \eqref{GMSW_review_flux}. As expected, it has exactly the same structure
as $\overline G_4$ in \eqref{overlineG4_4d}.

The fact that the topology of the internal space $M_6$
in the GMSW solutions matches exactly
with the topology of $M_6$ in our UV setup
is a strong hint that the GMSW solution provides
the gravity dual to the field theory setups
we discussed in section  \ref{4dsection}.
Furthermore, the GMSW solutions provide evidence
for the fact that the 4d construction yields a non-trivial
IR fixed point, at least at large $N$.

In the remainder of this section we perform two
quantitative checks of our proposed field theory interpretation
of the GMSW solutions. Before entering the details of the computation,
let us briefly discuss our stategy.


On the field theory side, 
the inflow anomaly polynomial \eqref{total_inflow} is expected to be exact in $N$,
but to contain both the anomalies of the interacting SCFT of interest
and of decoupled sectors. It is natural to assume that the decoupled sectors
do not contribute to the leading order $N^3$. As a result, from \eqref{total_inflow}
we can safely extract the anomaly polynomial
for the interacting SCFT at large $N$.
We then perform $a$-maximization at large $N$ in order to identify
which linear combination of $U(1)_\psi$, $U(1)_{\rm N,S}$ is the
superconformal R-symmetry.
Once the latter is determined, its 't Hooft anomaly coefficients
give us the central charge $c$ and   the flavor central charge $B$
for the $SO(3)_\varphi$ symmetry originating from isometries of $S^2_\varphi$.
The quantities $c$ and $B$ can also be computed holographically
in the GMSW solutions. This supergravity computation is reported in
appendix \ref{sugra_app}. We find a perfect agreement with the
field theory results.



Let us discuss in greater detail the field theory derivation
of the quantities $c$, $B$.
The first step is simply to isolate the leading terms in \eqref{total_inflow}
at large $N$,
\begin{align} \label{large_N_poly}
I_6^\text{SCFT, large $N$}
& =
-\frac{2 \,  N^2 \,  \left( \chi   N    +N_{\rm N} \right) \left(   
   \chi   N - N_{\rm S} \right) \left(  \chi   N
   +N_{\rm N} - N_{\rm S}  \right)}{\left(2 \chi N  
   +N_{\rm N} - N_{\rm S} \right){}^2}
 \, \bigg[  \frac{ F^\psi}{2 \pi} \bigg] ^2 \, 
\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
\nn \\
& + \frac{2  \, N^2 \,   N_{\rm N}  \left(N_{\rm N} + \chi N
   \right) }{2 \chi N
   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi}{2\pi} \, \frac{F^\mathrm N}{2\pi} \, \bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
   + \frac{2  \, N^2 \,   N_{\rm S}
   \left(N_{\rm S} - \chi N \right) }{2 \chi N
   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi }{2\pi} \, \frac{ F^\mathrm S }{2\pi} \, 
\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
\nn \\
& + \bigg(  N^2 \, N_\mathrm N   + \frac 23  \chi N^3 \bigg) \,  \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^3
+ \bigg( -  N^2 \, N_\mathrm S   + \frac 23  \chi N^3 \bigg) \, 
 \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^3
 \nn \\
& + N^2 \, N_\mathrm S \, \frac{ F^{\rm S} }{2\pi} \, 
 \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^2
- N^2 \, N_\mathrm N    \, \frac{ F^{\rm N} }{2\pi} \, 
 \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^2
\nn \\
&  +  
\frac{N^2 \left(\chi^2 N^2 
-3 \,
   N_{\rm N} N_{\rm S}+2 \,  \chi N ( N_{\rm N}  - N_{\rm S}) \right)}{6
   \left(2 \chi N +N_{\rm N} - N_{\rm S}\right)}
 \, \frac{F^\psi }{2\pi}\, p_1(SO(3)_\varphi)
   \nn \\
& - \frac 14 \, N^2 \, \bigg(N_{\rm N} \, \frac{F^{\rm N}  }{2\pi}
- N_{\rm S} \, \frac{ F^{\rm S} }{2\pi} \bigg)   \, p_1(SO(3)_\varphi)   \ .
\end{align}
%\begin{align} \label{large_N_poly}
%I_6^\text{SCFT, large $N$}
%& =
%-\frac{2 \,  N \,  \left(N   \chi +N_{\rm N} \right) \left(N  
%   \chi - N_{\rm S} \right) \left(N \chi
%   +N_{\rm N} - N_{\rm S}  \right)}{\left(2 N \chi
%   +N_{\rm N} - N_{\rm S} \right){}^2}
% \, \bigg[  \frac{ F^\psi}{2 \pi} \bigg] ^2 \, 
%\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
%\nn \\
%& + \frac{2  \,   N_{\rm N}  \left(N_{\rm N} + N \chi
%   \right) }{2 N \chi
%   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi}{2\pi} \, \frac{F^\mathrm N}{2\pi} \, \bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
%   + \frac{2   \,   N_{\rm S}
%   \left(N_{\rm S} - N \chi \right) }{2 N \chi
%   +N_{\rm N} - N_{\rm S}} \, \frac{ F^\psi }{2\pi} \, \frac{ F^\mathrm S }{2\pi} \, 
%\bigg( \frac{F^{\rm N} }{2\pi} + \frac{ F^{\rm S} }{2\pi} \bigg)
%\nn \\
%& + \bigg(  \frac{N_{\rm N}}{N} + \frac 23  \chi \bigg) \,  \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^3
%+ \bigg( - \frac{N_{\rm S}}{N} + \frac 23  \chi \bigg) \, 
% \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^3
%+ \frac{N_{\rm S}}{N} \, \frac{ F^{\rm S} }{2\pi} \, 
% \bigg[  \frac{ F^\mathrm N}{2 \pi} \bigg] ^2
%- \frac{N_{\rm N}}{N} \,  \, \frac{ F^{\rm N} }{2\pi} \, 
% \bigg[  \frac{ F^\mathrm S}{2 \pi} \bigg] ^2
%\nn \\
%&  +  
%\frac{N^2 \left(N^2 \chi ^2
%-3 \,
%   N_{\rm N} N_{\rm S}+2 \,  N \chi ( N_{\rm N}  - N_{\rm S}) \right)}{6
%   \left(2 N \chi +N_{\rm N} - N_{\rm S}\right)}
% \, \frac{F^\psi }{2\pi}\, p_1(SO(3)_\varphi)
%   \nn \\
%& - \frac 14 \, N \, \bigg(N_{\rm N} \, \frac{F^{\rm N}  }{2\pi}
%- N_{\rm S} \, \frac{ F^{\rm S} }{2\pi} \bigg)   \, p_1(SO(3)_\varphi)   \ .
%\end{align}
Next, we perform $a$-maximization.
The trial superconformal R-symmetry is a linear combination of $U(1)_\psi$
 with $U(1)_{\rm N,S}$, parametrized as
\beq \label{generator_shift}
R = T_\psi +   s^\mathrm N \, T_\mathrm N +   s^\mathrm S \, T_\mathrm S \ ,
\eeq
where $T_\psi$, $T_{\rm N,S}$ denote 
the   generators of $U(1)_\psi$, $U(1)_{\rm N,S}$,
and 
$  s^{\rm N,S}$ are parameters   to be fixed. 
At leading order at large $N$,
\beq
I_6^\text{SCFT} = \frac 16 \, {\rm tr} \, R^3 \, \bigg[ 
\frac{F^R}{2\pi}
\bigg]^3 \ , \qquad
a = c = \frac{9}{32} \,  {\rm tr} \, R^3 \ , 
\qquad \qquad \text{(large $N$)}
\eeq
where $F^R$ is the background curvature
for the superconformal R-symmetry.
At the level of the anomaly polynomial,
\eqref{generator_shift} is equivalent to 
the replacements
\beq \label{replacements}
F^\psi \rightarrow F^R \ , \qquad
F^{\rm N,S} \rightarrow   s^{\rm N,S} \, F^R \ ,
\eeq
where $F^R$ denotes the background curvature
for the superconformal R-symmetry.
It follows that $a$-maximization at large $N$
can be carried out
by taking \eqref{large_N_poly}, performing the replacements
\eqref{replacements}, and maximizing the coefficient of $(F^R)^3$ with respect to the parameters
$  s^{\rm N,S}$.
The result of this computation is
most conveniently written in terms of the 
quantities
\beq
N_\Sigma = - \frac 12 ( N \, \chi + N_\mathrm N - N_\mathrm S  ) \ , \qquad
M = \frac 12 (N_\mathrm N + N_\mathrm S) \ .
\eeq
The central charge reads
\begin{align} \label{largeN_c}
c & = 
\frac{9 N^2   N_{\Sigma }^2  
   \,      \Big[ \chi^2 N^2   + 2 \chi   N    N_\Sigma  + 4 \, N_\Sigma^2 - 3  M^2 \Big]^{3/2}    
   }{4 \left(3 M^2+2 \chi N    N_{\Sigma
   }\right){}^2}
   \nn \\
   & -\frac{9 N^2 N_{\Sigma }^2 \left(2 N_{\Sigma }+\chi N   \right)
   \left(2 \chi^2 N^2  +2 \chi N    N_{\Sigma }+8 N_{\Sigma }^2  -9 M^2 \right)}{8
   \left(3 M^2+2 \chi N    N_{\Sigma }\right){}^2} \ .
\end{align}
For completeness, let us also record the values of the 
parameters $s^{\rm N,S}$,
\begin{align} \label{s_parameters}
s^{\rm N,S} & = 
\frac{  2 \chi^2 N^2 N_\Sigma - 8 N_\Sigma^3  \pm M \, ( \chi^2 N^2 - 4 \chi NN_\Sigma - 4 N_\Sigma^2 )  \mp 6 M^3 }{ 2 \, (\chi N - 2 N_\Sigma) \, ( 3M^2 + 2 \chi N N_\Sigma ) }
\nn \\
& - \frac{2 N_\Sigma \mp M}{2 \, ( 3M^2 + 2 \chi N N_\Sigma)} \, \sqrt{  \chi^2 N^2   + 2 \chi   N    N_\Sigma  + 4 \, N_\Sigma^2 - 3  M^2   }  \ .
\end{align}
%\begin{align} \label{s_parameters}
%s^\mathrm N & = 
%\frac{   -6 M^3+M N^2 \chi ^2-4 M N \chi  N_{\Sigma }-4 M N_{\Sigma }^2+2 N^2
%   \chi ^2 N_{\Sigma }-8 N_{\Sigma }^3  }{2 \left(N \chi -2 N_{\Sigma }\right)
%   \left(3 M^2+2 N \chi  N_{\Sigma }\right)}
%   \nn \\
%   & -\frac{ M+2
%   N_{\Sigma } }{2 \left(3 M^2+2 N \chi  N_{\Sigma }\right)} \, 
%      \sqrt{  \chi^2 N^2   + 2 \chi   N    N_\Sigma  + 4 \, N_\Sigma^2 - 3  M^2   }  \  , \nn \\
% s^\mathrm S & =   
%-\frac{ -6 M^3+M N^2 \chi ^2-4 M N \chi  N_{\Sigma }-4
%   M N_{\Sigma }^2-2 N^2 \chi ^2 N_{\Sigma }+8 N_{\Sigma }^3 }{2 \left(N \chi
%   -2 N_{\Sigma }\right) \left(3 M^2+2 N \chi  N_{\Sigma }\right)}
%   \nn \\
%   & + \frac{ M-2 N_{\Sigma } }{2 \left(3 M^2+2 N \chi 
%   N_{\Sigma }\right)} \,       \sqrt{  \chi^2 N^2   + 2 \chi   N    N_\Sigma  + 4 \, N_\Sigma^2 - 3  M^2   }   \ .
%\end{align}

Let us now discuss the flavor central charge $B$
for the $SO(3)_\varphi$ symmetry.
The quantity $B$ appears in the 2-point function
of two $SO(3)_\varphi$ symmetry currents.
For its normalization, we follow the conventions of \cite{sdsds}.
The superconformal algebra relates $B$ to the 't Hooft anomaly
between the superconformal R-symmetry and $SO(3)_\varphi$ \cite{sdsd}.
Let us define the 't Hooft anomaly coefficient
$\cA_{SO(3)_\varphi}$ by
\beq
I_6^{\rm SCFT} = \cA_{SO(3)_\varphi} \, \frac{F^R}{2\pi} \, p_1(SO(3)_\varphi) + \dots
\eeq
We then have
\beq
B = 4 \, \cA_{SO(3)_\varphi} \ .
\eeq
The quantity $\cA_{SO(3)_\varphi}$ is extracted from 
\eqref{large_N_poly} by performing the replacements
\eqref{replacements} and using \eqref{s_parameters}.
The result for $B$ then reads
\begin{align} \label{field_theory_B}
B  & = 
\frac{N^2 \left( 4 \chi^2 N^2   N_{\Sigma }+12 \chi N
      N_{\Sigma }^2+24 N_{\Sigma }^3
   -30 M^2 N_{\Sigma }-9 \chi M^2 N  \right)}{6 \left(3 M^2+2\chi  N    N_{\Sigma
   }\right)}
   \nn \\
   & -\frac{N^2   \left( \chi N    N_{\Sigma }+2 N_{\Sigma
   }^2  -M^2 \right)}{  3 M^2+2 \chi N    N_{\Sigma } } \, 
      \sqrt{   \chi^2 N^2   + 2 \chi   N    N_\Sigma  + 4 \, N_\Sigma^2 - 3  M^2   }  \ .
\end{align}
%\begin{align} \label{field_theory_B}
%B  & = 
%\frac{N^2 \left(-30 M^2 N_{\Sigma }-9 M^2 N \chi +4 N^2 \chi ^2 N_{\Sigma }+12 N
%   \chi  N_{\Sigma }^2+24 N_{\Sigma }^3\right)}{6 \left(3 M^2+2 N \chi  N_{\Sigma
%   }\right)}
%   \nn \\
%   & -\frac{N^2   \left(-M^2+N \chi  N_{\Sigma }+2 N_{\Sigma
%   }^2\right)}{  3 M^2+2 N \chi  N_{\Sigma } } \, 
%      \sqrt{  N^2 \, \chi^2 + 2 \, N \, N_\Sigma \, \chi + 4 \, N_\Sigma^2 - 3 \, M^2  }  \ .
%\end{align}

For definiteness, the supergravity computation of appendix \ref{sugra_app}
is performed in the case in which the Riemann surface has genus $g \ge 2$ and
the flux parameter $M$ is set to zero.
The results for $c$ and $B$ are given in \eqref{sugra_c}, \eqref{sugra_B}
in terms of the quantity $\tilde r = - 2 N_\Sigma /(N \chi)$.
They agree perfectly with \eqref{largeN_c}, \eqref{field_theory_B},
respectively.


%
%
%
%\newpage
%
%with the warp factor $\lambda$ and the metric functions
%$F_\varphi$, $F_\Sigma$, $\cos \zeta$
%given by\footnote{The coordinate $y$ in \cite{Gauntlett:2004zh}
%is identified with the coordinate $\mu$ here.
%Moreover, compared to \cite{Gauntlett:2004zh}, we have flipped the sign of $\psi$. For simplicity, we have set the $AdS_5$ scale to $1$, so that the Ricci scalar of $AdS_5$ is $R = -20 $.}
%\begin{align}
%e^{6\lambda} &= 
%\frac{2   \left(a_\varphi -    \mu^2\right) \left(a_\Sigma  - k \, 
%   \mu^2\right)}{a_\Sigma   + k \,  a_\varphi  +2  \, \mu \,  \left( 3 \, a_0 + k \, \mu
%    \right)}
%    \ , \nn \\ 
%F_{\varphi}   &= \frac 13 (a_\varphi -   \mu^2)    \ , \qquad
%F_{\Sigma}   = \frac 13 (a_\Sigma  - k\,  \mu^2)    \ , \qquad
%e^{3\lambda} \, \sin \zeta = 2  \mu  \ .
%\end{align}
%In the above expressions, $a_\varphi$, $a_\Sigma$,
%$a_0$ are constant parameters.
%The quantity $k$ is the curvature of the Riemann surface 
%$\Sigma_g$, with $k = +1$ for $g = 0$ and $k = -1$
%for $g>1$.
%The 1-form $\widehat D\psi$ was given in \eqref{hatDpsi}.
%%and satisfies
%%\beq
%%d \frac{\widehat D\psi}{2\pi} = - 2 \bigg[ V_2^\varphi + V_2^\Sigma \bigg] \ ,
%%\eeq
%%with the volume forms $V_2^\varphi$, $V_2^\Sigma$
%%on $S^2_\varphi$, $\Sigma_g$ normalized
%%as in \eqref{Vnormalization}.
%%In this section 
%%
%The range $[\mu_\mathrm S, \mu_\mathrm S]$ of the interval coordinate $\mu$
%is specified by the zeros of $\cos \zeta$.
%On the entire interval $[\mu_\mathrm S, \mu_\mathrm S]$
%the warp factor $e^{2\lambda}$ and the metric
%functions $F_\varphi$, $F_\Sigma$
%are strictly positive. The interval $\mu$ and the angle
%$\psi$ combine into a topological $S^2_{\mu\psi}$,
%which is free of conical singularities 
%at $\mu_{\mathrm N,S}$, where $S^1_\psi$
%shrinks.
%Topologically, \eqref{IRgeometry} thus describes
%a fibration of $S^2_{\mu \psi}$ on $S^2_\varphi \times \Sigma_g$.
%This fits with our UV picture, in which
%$M_4$, which is an $S^2$ bundle over $S^2$,
%is fibered over the Riemann surface.
%
% 
%
%
%
%The geometry $\eqref{IRgeometry}$ is supported
%by a $G_4$-flux configuration
%of exactly the same form as $\overline G_4$ in \eqref{overlineG4_4d}.
%In the backreacted solution, the functions
%$\gamma_\varphi$, $\gamma_\Sigma$
%are  rational functions of $\mu$.
%Their explicit expression can be found in \cite{Gauntlett:2004zh},
%but is not needed in this work.
%Notice that the three parameters $a_\varphi$, $a_\Sigma$,
%$a_0$ are in 1-to-1 correspondence
%with the three independent flux quanta
%$N$, $N_\mathrm N$, $N_\mathrm S$ \cite{Gauntlett:2006ai}.
%
%
%
%The fact that the topology of the internal space $M_6$
%in the GMSW solutions matches exactly
%with the topology of $M_6$ in our UV setup
%is a strong hint that the GMSW solution provides
%the gravity dual to the field theory setups
%we discussed in section  \ref{4dsection}.
%Furthermore, the GMSW solutions provide evidence
%for the fact that the 4d construction yields a non-trivial
%IR fixed point, at least at large $N$.
%
%A quantitative check of our proposal 
%is the match of the central charge $c$ computed
%holographically with the line element \eqref{IRgeometry}
%and the central charge obtained on the field theory
%side via $a$-maximization at large $N$.
%
%The inflow anomaly polynomial of the field theory
%is given in \eqref{total_inflow}. While inflow is exact in $N$,
%\eqref{total_inflow} contains both the contributions
%of the interacting SCFT we want to study,
%as well as the contributions of modes that decouple
%in the IR. We expect the decoupling modes to 
%have anomalies 
%that are subleading in $N$. As a result, if we focus
%on the leading terms in the large-$N$ expansion, 
%we can write
%\begin{align} \label{large_N_poly}
%(2\pi)^3 \, I_6^\text{SCFT, large $N$} & = - (2\pi)^3 \, I_6^\text{inflow, large $N$} 
%  \\
%&= 
%-\frac{2 \,  N \,  \left(N   \chi +N_{\rm N} \right) \left(N  
%   \chi - N_{\rm S} \right) \left(N \chi
%   +N_{\rm N} - N_{\rm S}  \right)}{\left(2 N \chi
%   +N_{\rm N} - N_{\rm S} \right){}^2}
%\, (F^\psi)^2 \, ( F^{\rm N}  + F^{\rm S} )
%\nn \\
%& + \frac{2  \left(F^{\rm S} N_{\rm S}
%   \left(N_{\rm S} - N \chi \right)+F^{\rm N} N_{\rm N}  \left(N_{\rm N} + N \chi
%   \right)\right)}{2 N \chi
%   +N_{\rm N} - N_{\rm S}} \, F^\psi \, \left(F^{\rm N}+F^{\rm S}\right)
%\nn \\
%& + \bigg(  \frac{N_{\rm N}}{N} + \frac 23  \chi \bigg) \, (F^{\rm N})^3
%+ \bigg( - \frac{N_{\rm S}}{N} + \frac 23  \chi \bigg) \, (F^{\rm S})^3
%+ \frac{N_{\rm S}}{N} \, F^{\rm S} \, (F^{\rm N})^2
%- \frac{N_{\rm N}}{N} \, F^{\rm N} \, (F^{\rm S})^2
%\ . \nn
%\end{align}
%The large-$N$ limit is taken by letting the fluxes $N_{\rm N,S}$ and the background curvatures $F^{\rm N,S}$
%scale like $N$. Furthermore, we have turned off the background
%curvature for the non-Abelian symmetry $SO(3)_\varphi$,
%since it cannot play a role in $a$-maximization.
%
%
%
%
%The superconformal R-symmetry is a mixture of $U(1)_\psi$
% with $U(1)_{\rm N,S}$, parametrized as
%\beq \label{generator_shift}
%R = t_\psi +   s_\mathrm N \, t_\mathrm N +   s_\mathrm S \, t_\mathrm S \ ,
%\eeq
%where $t_\psi$, $t_{\rm N,S}$ denote 
%the   generators of $U(1)_\psi$, $U(1)_{\rm N,S}$.
%The parameters $  s_{\rm N,S}$ are fixed
%by $a$-maximization \cite{Intriligator:2003jj}.
%At leading order at large $N$,
%\beq
%I_6^\text{SCFT} = \frac 16 \, {\rm tr} \, R^3 \, \bigg[ 
%\frac{F^R}{2\pi}
%\bigg]^3 \ , \qquad
%a = c = \frac{9}{32} \,  {\rm tr} \, R^3 \ , 
%\qquad \qquad \text{(large $N$)}
%\eeq
%where $F^R$ is the background curvature
%for the superconformal R-symmetry.
%At the level of the anomaly polynomial,
%\eqref{generator_shift} is equivalent to 
%the replacements
%\beq \label{replacements}
%F^\psi \rightarrow F^R \ , \qquad
%F^{\rm N,S} \rightarrow   s_{\rm N,S} \, F^R \ ,
%\eeq
%where $F^R$ denotes the background curvature
%for the superconformal R-symmetry.
%It follows that $a$-maximization at large $N$
%can be carried out
%by taking \eqref{large_N_poly}, performing the replacements
%\eqref{replacements}, and maximizing the coefficient of $(F^R)^3$ with respect to the parameters
%$  s^{\rm N,S}$.
%The result of this computation is
%\begin{align} \label{leading_c}
%c & = \frac 98 \, \frac{N^2 (N\chi + N_{\rm N} - N_{\rm S})^2
%\, \Big[ 
%4 N^2 \chi^2 + 4 N\chi (N_{\rm N} - N_{\rm S}) 
%+ N^2_{\rm N} - 14 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%\Big]^{3/2}
%}{\Big[    4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})   \Big]^2}
%  \\
%& - \frac 98 \, \frac{
%N^2 (N\chi + N_{\rm N} - N_{\rm S})^2 (N_{\rm N} - N_{\rm S}) \, 
%\Big[
%N_{\rm N}^2 + 34 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%- 12 N\chi (N_{\rm N} - N_{\rm S}) - 12 N^2 \chi^2 
%\Big]
%}{\Big[    4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})   \Big]^2} \ . \nn
%\end{align}
%This expression matches exactly with the holographic
%results of \cite{Gauntlett:2006ai}, where an explicit expression
%for $c$ is given in the case in which the Riemann surface is a sphere and $N^{\rm N} + N^{\rm S} = 0$.
%
%
%Knowledge of the inflow anomaly polynomial
%\eqref{total_inflow}, combined with some mild
%assumptions about the contribution of decoupling modes,
%allows us to obtain a prediction for the leading $1/N$
%correction to \eqref{leading_c}. More precisely,
%let us assume that the anomalies of decoupling modes
%do not have any $\cO(N)$ contribution,
%so that the identification $I_6^{\rm SCFT} = - I_6^{\rm inflow}$ holds both at $\cO(N^3)$ and $\cO(N)$.
%Under this assumption, we can perform $a$-maximization
%order by order in $1/N$, using \eqref{total_inflow}
%as input, and compute $c$ as an expansion in $1/N$.
%As expected, the first non-zero correction to the leading
%value of $c$ comes at order $1/N^2$, and is given by
%\begin{align}
%\Delta c &  =
%- \frac{11}{8} \, \frac{
%N\chi (N\chi + N_{\rm N} - N_{\rm S}) \,
%\Big[ 
%4 N^2 \chi^2 + 4 N\chi (N_{\rm N} - N_{\rm S}) 
%+ N^2_{\rm N} - 14 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%\Big]^{1/2}
%}{
% 4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})  
%}
%\nn \\
%&
% - \frac 38 \,
%\frac{ (N_{\rm N} - N_{\rm S}) \, \Big[
%(N_{\rm N} + N_{\rm S})^2 + 6 N\chi (N_{\rm N} - N_{\rm S}) + 6N^2 \chi^2
%\Big]  }{
% 4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})  
%} \ .
%\end{align}
%It would be interesting to perform a holographic check of this
%result. We leave this point for future investigation. 
% 
%
%
%
%************
%
%************
%
%\subsection{Brief review of the solutions}  
%
%In this appendix we review a class of  M-theory 
%solutions with 4d $\cN = 1$ superconformal symmetry,  first described in GMSW \cite{Gauntlett:2004zh}.
%The 11d metric reads
%\begin{align} \label{GMSW_review_metric}
%ds^2_{11} & = L^2 \, e^{2\lambda} \, \Big[ ds^2(AdS_5) 
%+  ds^2(M_6) \Big] \ ,  \nn  \\
%ds^2(M_6) & = e^{-6\lambda} \Big[ F_1 \, d  s^2(C_1)
%+ F_2 \, d  s^2(C_2) \Big]
%+ \frac{e^{-6\lambda}}{\cos^2\zeta} dy^2
%+ \frac{\cos^2 \zeta}{9} D\psi^2 \ , \nn \\
%dD\psi &= - \chi_1 \, V_{C_2} - \chi_2 \, V_{C_2} \ .  
%\end{align}
%The constant $L$ is the overall length scale of the solution.
%The metric on $AdS_5$ is normalized in such a way that 
%the Ricci scalar is $R_{\rm AdS_5} = -20$.
%The spaces $C_1$, $C_2$ are two Riemann surfaces, of arbitrary genus.
%If $C_i$, $i = 1,2$, is not a torus, the metric $ds^2(C_i)$
%is normalized so that the Ricci scalar is $R_{C_i}= 2 \, k_i$,
%with $k_i = \pm 1$. The symbol $\chi_i$ denotes the Euler
%characteristic of $C_i$,
%while $V_{C_i}$ is proportional to the volume form on $C_i$.
%If $C_i$ is not a torus, $V_{C_i}$ is normalized according to
%$\int_{C_i} V_{C_i}  = 2\pi$,
%with no sum over $i$.
%Notice that, compared to \cite{Gauntlett:2004zh},
%we have reversed the sign of $\psi$.
%
%The quantities $\lambda$, $F_i$ 
%depend on $y$ only and are given by
%\begin{align}
%e^{6\lambda} &= 
%\frac{2   \left(a_1-k_1 \,  y^2\right) \left(a_2-k_2 \ 
%   y^2\right)}{a_2  \, k_1+a_1 \,  k_2+2  \, y \, k_1 \, k_2 \left(  y - 3 \, \gamma_0
%    \right)}
%    \ , \qquad 
%F_i   = \frac 13 (a_i - k_i \,  y^2)    \ ,
%\end{align}
%where  $a_i$, $\gamma_0$ are constants.
%The quantity $\zeta \in [0, \pi/2]$   is determined by
%\beq
%e^{3\lambda} \, \sin \zeta = 2  \, y \  \ .
%\eeq
%The $G_4$ flux takes the form
%\beq \label{GMSW_review_flux}
%G_4 = L^3 \, \Big[  
%(d\gamma_1 \, V_{C_1} + d\gamma_2 \, V_{C_2} )\, D\psi
%- (\chi_1 \, \gamma_2 + \chi_2 \, \gamma_1 +
%\chi_1 \, \chi_2 \, \gamma_0) \, V_{C_1} \, V_{C_2}
%\Big] \ ,
%\eeq
%with the functions $\gamma_i$  given as
%\begin{align} \label{fi_expr}
%\gamma_1 & = \frac{
%2  \, a_2 \,  k_1 \,  k_2 \,  y - 6  \, a_2 \,  k_1 \, k_2 \, \gamma_0 +a_1 \,  y+k_1  \, y^3
%}{
%9  \, k_1 \, k_2 \,   \left(a_2 - k_2 \,  y^2 \right)
%}  \, \chi_1
%\ , \nn \\
%\gamma_2 & = \frac{
%2 \,  a_1 \,  k_1 \,  k_2 \,  y -  6  \, a_1 \, k_1 \, k_2 \, \gamma_0 +a_2 \,  y+k_2 \,  y^3
%}{
%9 \, k_1 \, k_2 \,  \left(a_1 - k_1 \, y^2\right)
%}  \, \chi_2 
%\ .
%\end{align}
%We are adopting conventions in which the quantization of $G_4$ flux 
%reads
%\beq \label{G4_quantization_convention}
%\int_{\cC_4} \frac{G_4}{(2\pi \ell_p)^3} \in \mathbb Z \ ,
%\eeq
%where $\cC_4$ is a 4-cycle and $\ell_p$ is the 11d Planck length.
%
%Let us stress that, in this work, we only consider GMSW
%solutions of the form \eqref{GMSW_review_metric},
%\eqref{GMSW_review_flux}
% in which none
%of the Riemann surfaces $C_i$ is a torus,
%so that $k_i \neq 0$.
%According to the analysis of \cite{Gauntlett:2004zh},
%in order to a have a regular solution 
%at least one of the two Riemann surfaces must be a sphere.
%We associate the label 1 to this sphere, 
%while the label 2 is reserved to a Riemann surface of genus $g$,
%with $g = 0$ or $g \ge 2$,
%\beq
%C_1 = S^2 \ , \qquad
%C_2 = \Sigma_g   \ .
%\eeq
%We should emphasize that the 4-form $V_4$ in \eqref{GMSW_V4}
%is understood to have integral fluxes
%along 4-cycles. It follows from \eqref{G4_quantization_convention}
%that the relation between $V_4$ and $G_4$ is
%\beq
%V_4 = \frac{G_4}{(2\pi \ell_p)^3} \ .
%\eeq 
%In the main text, we parametrized $V_4$ by writing
%\beq
%V_4 = 
%\bigg[  d\gamma_\Sigma \, \frac{V_\Sigma}{2\pi}
%+ d\gamma_{S^2} \, \frac{V_{S^2}}{2\pi} \bigg] \, \frac{D\psi}{2\pi}
%- \Big[ 2\, \gamma_\Sigma + \chi  \, \gamma_{S^2}   \Big] \,
%\frac{V_\Sigma}{2\pi}  \, \frac{V_{ S^2}}{2\pi}  \ .
%\eeq
%Comparison with \eqref{GMSW_review_flux} gives the identifications
%\beq \label{fi_identifications}
%\gamma_{S^2} = \frac{L^3}{ 2\pi \,  \ell_p^3} \, (\gamma_1 + s_1) \ , \qquad
%\gamma_{\Sigma} = \frac{L^3}{ 2\pi \,  \ell_p^3} \, (\gamma_2 + s_2 ) \ ,
%\qquad
%2 \, s_2 + \chi \, s_1  = 2 \, \chi \, \gamma_0 \ ,
%\eeq
%where the constants $s_{1,2}$ 
%can be chosen at will. In the text, 
%this ambiguity in the precise definition of $\gamma_\Sigma$, $\gamma_{S^2}$
%is resolved upon construction of $E_4$, when the condition
% \eqref{omegaI_condition} is enforced.
%
%
%%As a result, we identify the functions 
%%$f_{S^2}$, $f_\Sigma$ in $V_4$ with $f_1$, $f_2$ 
%%in \eqref{fi_expr} according to
%%\beq \label{fi_identifications}
%%f_{S^2} = \frac{f_1}{(2\pi \ell_p)^3} \ , \qquad
%%f_{\Sigma} = \frac{f_2}{(2\pi \ell_p)^3}  \ .
%%\eeq
%% We also have the identifications
%%\beq
%%N_1 := \int_{C_1 \times S^2_{y\psi}} \frac{G_4}{(2 \pi \ell_p)^3}
%%= \int_{S^2 \times S^2_{y\psi}} V_4 =: N_{S^2} \ , \quad
%%N_2 := \int_{C_2 \times S^2_{y\psi}} \frac{G_4}{(2 \pi \ell_p)^3}
%%= \int_{\Sigma_g \times S^2_{y\psi}} V_4 =: N_{\Sigma}
%%\eeq 
%%
%%
%%
%%
%%Let us now report in greater detail some properties of the
%%solutions with $f_0 = 0$, which are symmetric under
%%the reflection $y \leftrightarrow -y$.
%%It is convenient to distinguish the case in which $\Sigma_g$
%%is a sphere ($k_2 =+1$) and the case in which it is a higher-genus surface
%%($k_2 = -1$).
%%Our review also includes results first obtained in \cite{Gauntlett:2006ai}.
%%
%%
%%\paragraph{The case $k_2 = +1$.}
%%To have a well-behaved solution, we need
%%\beq
%%a_1 >0 \ , \qquad
%%a_2 >0 \ .
%%\eeq
%%The range of the $y$ coordinate is $[- y_{\rm max}, y_{\rm max}]$,
%%with
%%\beq
%%y_{\rm max}^2 = - \frac 12 (a_1 + a_2) + \frac12 \, \sqrt{
%%(a_1 + a_2)^2 + \frac 43 \, a_1 \, a_2
%%} \ .
%%\eeq
%%The ratio $a_2/a_1$ is determined by the flux quanta $N_1$, $N_2$,
%%\beq
%%\frac{a_2}{a_1} = \frac{2 \, r^2  - r  + 2 + 2 \, (r -1) \, \sqrt{1 + r + r^2}}{3 \, r} \ , \qquad
%%r := \frac{N_2}{N_1} \ .
%%\eeq
%%The Planck length can be written in terms of $L$ and $N_1$ or $N_2$ as
%%\beq
%%L^{-3} \, \ell_p^3 = \frac{2 \, y_{\rm max} \, (a_1 + 2 \, a_2  + y_{\rm max}^2)}{
%%9 \, \pi \, N_1 \, (a_2 - y_{\rm max}^2)
%%}
%%= \frac{2 \, y_{\rm max} \, (2 \, a_1 + a_2  + y_{\rm max}^2)}{
%%9 \, \pi \, N_2 \, (a_1 - y_{\rm max}^2)
%%} \ .
%%\eeq
%%The central charge $c$ of the dual SCFT
%%is extracted from the volume of the internal space,
%%\beq \label{holo_c}
%%c = \frac{1}{2 \, (2\pi)^6} \, L^{-9} \, \ell_p^9 \int_{M_6} e^{9\lambda} \, {\rm vol}_{M_6} \ ,
%%\eeq
%%where ${\rm vol}_{M_6}$ is the
%%volume form associated to the metric $ds^2(M_6)$ in \eqref{GMSW_review_metric}.
%%After a few manipulations, including denesting a nested square root,
%%we obtain 
%%\beq \label{sphere_central_charge}
%%c = \frac 98 \, \bigg[
%%( N_1 ^2 + N_1 \,  N_2  + N_2^2 )^{3/2}
%%- \frac 12 \, (N_1 + N_2) (2 \, N_1^2 + N_1 \, N_2 + 2 \, N_2^2)
%%\bigg] \ .
%%\eeq
%%
%%
%%
%%\paragraph{The case $k_2 = -1$.}
%%To have a well-behaved solution, in this case we need
%%\beq
%%0 < 3 \, a_1 < a_2  \ .
%%\eeq
%%The range of the $y$ coordinate is $[- y_{\rm max}, y_{\rm max}]$,
%%with
%%\beq
%%y_{\rm max}^2 =  \frac 12 (a_1 - a_2) - \frac12 \, \sqrt{
%%(a_1 - a_2)^2 - \frac 43 \, a_1 \, a_2
%%} \ .
%%\eeq
%%The ratio $a_2/a_1$ is determined by the flux quanta $N_1$, $N_2$,
%%\beq
%%\frac{a_2}{a_1} = 
%%\frac{ 2 \, r^2 + r \, + 2 \, + 2 \, \sqrt{1 + r + r^3 + r^4} }{3 \, r} \ , \qquad
%%r := \frac{2 \, N_2}{|\chi_2| \, N_1}
%%\ .
%%\eeq
%%We notice that $a_2 > 3 \, a_1$ implies
%%\beq
%%2 \, N_2 > |\chi_2| \, N_1  \ .
%%\eeq
%%The Planck length can be written in terms of $L$ and $N_1$ or $N_2$ as
%%\beq
%%L^{-3} \, \ell_p^3 = \frac{2 \, y_{\rm max} \, (2 \, a_2 - a_1  - y_{\rm max}^2)}{
%%9 \, \pi \, N_1 \, (a_2 + y_{\rm max}^2)
%%}
%%= \frac{|\chi_2|}{2} \frac{2 \, y_{\rm max} \, (a_2 - 2 \, a_1    - y_{\rm max}^2)}{
%%9 \, \pi \, N_2 \, (a_1 - y_{\rm max}^2)
%%} \ .
%%\eeq
%%The central charge $c$ is again computed from \eqref{holo_c}.
%%After some manipulations, similar to those of the case $k_2 = 1$,
%%it can be cast in the form
%%\beq \label{final_central_charge}
%%c = \frac {9}{16} \frac{1}{\chi_2^2} \bigg[
%%  (4 \, N_2^2 + 2 N_1 \, N_2 \, \chi_2 +   N_1^2 \, \chi_2^2)^{3/2}
%%- (2 \, N_2 +   N_1 \, \chi_2 ) (
%%4 \, N_2^2 +   N_1 \, N_2 \, \chi_2  +  \, N_1^2 \, \chi_2^2
%%)
%%\bigg] \ .
%%\eeq
%%Notice that, if we continue this expression in $\chi_2$
%%from the negative value $\chi_2 = 2(1-g)$ appropriate for $\Sigma_g$
%%to the value $\chi_2 = +2$ corresponding to a 2-sphere, we find an agreement with the central charge \eqref{sphere_central_charge}
%%in the case $k_2 = 1$. 
%
%
%The holographic central charge for these solutions
%was analyzed in \cite{Gauntlett:2006ai},
%where the explicit value of $c$ is derived in the case $\gamma_0 = 0$,
%$\Sigma_g = S^2$. 
%In this situation, one verifies that 
%$N^{\rm N} = - N^{\rm S}$,
%or equivalently $M = 0$, see \eqref{north_and_south_fluxes}, \eqref{M_def}. 
%In the notation of \cite{Gauntlett:2006ai} the central charge reads
%\beq \label{their_c}
%c = \frac{3^{3/2}}{2^6} \, \frac{9 \, (z+1)^3 - (3 \, z^2 + 4 \, z + 3) \, \sqrt X}{z^{3/2}} \, 
%p^{3/2} \, q^{3/2} \, N^3 \ ,
%\eeq
%where the parameters $p$, $q$, $N$ are related to our quantities $N_{S^2}$,
%$N_\Sigma$ by $N_{S^2} = N \, p$, $N_\Sigma = N \, q$.
%The objects $X$, $z$ are defined as
%\beq
%X = 9 \, z^2 + 30 \, z + 9 \ , \qquad
%z = \frac{2 \, q^2 - p \, q + 2 p^2 - 2 \, (p-q) \, \sqrt{p^2 + p \,q  + q^2}}{3 \, p \, q} \ .
%\eeq
% In order to compare \eqref{their_c}  
%to the central charge \eqref{central_charge} inferred from the inflow anomaly polynomial,
%we need the following identity,
%valid for positive numbers $p$, $q$,
%\begin{align} \label{strange_identity}
%\left(
%2 \, p^2 - p \, q + 2 \, q^2 - 2 \, (p-q) \, \sqrt{p^2 + p \, q + q^2}
% \right)^{1/2}
% & = 
% q-p + \sqrt{p^2 + p  \, q + q^2}   \ .
%\end{align}
%With the help of \eqref{strange_identity},
%the central charge \eqref{their_c} can be rewritten as
%\beq
%c = - \frac{9}{16} \, N^3 \, (p + q) \, (2 \, p^2 + p \, q + 2 \, q^2)
%+ \frac 98 \, N^3 \, (p^2 + p \, q + q^2)^{3/2} \ ,
%\eeq
%which indeed matches \eqref{central_charge} for $\chi = 2$, $M = 0$.
%
%%
%%{\bf [What comes next is probably not needed anymore]}
%%
%%
%%We conclude this appendix by collecting some details
%%about the extremization of the inflow anomaly polynomial.
%%The quantity to extremize is $\int_{M_6} E_4^3$ with $E_4$
%%given in \eqref{E4_in_GMSW}.
%%The parameters we extremize on are the 
%%quantities that parametrize the gauging ambiguities
%%in going from $V_4$ in \eqref{GMSW_V4} to $E_4$ in \eqref{E4_in_GMSW}.
%%These parameters are $C_{S^2}$, $C_\Sigma$, $u$,
%%and the values of the function $H$ at the endpoints of the
%%$y$ interval, denoted $H^{\rm N}$ and $H^{\rm S}$. (The anomaly polynomial
%%is insensitive to the profile of $H$ in the interior of the $y$ interval.) 
%%We stress that 
%%$f_0$ and the values of  $f_{S^2}$, $f_\Sigma$
%%at the endpoints of the $y$ interval
%%are not considered free parameters, because 
%%they describe $V_4$ itself, rather than  its gauging.
%%Keeping fixed $f_0$, $f_{S^2}$, and $f_\Sigma$
%%guarantees that the three independent
%%flux quantum numbers $(N_{S^2}, N_\Sigma, M)$
%%are held fixed during extremization.
%%
%%
%%We have to set to zero the derivatives of $\int_{M_6} E_4^3$
%%with respect to $C_{S^2}$, $C_\Sigma$, $u$, $H^{\rm N}$, $H^{\rm S}$.
%%The resulting algebraic system of equations
%%admits four branches of solutions.
%%The first two branches are
%%\begin{align} \label{bad_solus}
%%H^{\rm N} &= H^{\rm S} = C \ , \nn \\
%%C_{S^2} &= - 2 \, C \pm \frac{N_{S^2}}{8\pi^2} - \frac 12 (f_{S^2}^{\rm N} + f_{S^2}^{\rm S}) \ , \nn \\
%%C_{\Sigma} &= - \chi \, C \mp \frac{N_{\Sigma}}{8\pi^2} - \frac 12 (f_{\Sigma}^{\rm N} + f_{\Sigma}^{\rm S}) \ , \nn \\
%%u & = - C \ ,
%%\end{align}
%%where $C$ is an arbitrary constant. It is related to the redundancy in the parametrization
%%of $E_4$ discussed under \eqref{omegapsi_solu}.
%%The solutions \eqref{bad_solus} are not acceptable,
%%because, if   plugged back into $\int_{M_6} E_4^3$, they give zero.
%%
%%The other two solutions take the following form,
%%\begin{align} \label{good_solus}
%%H^{\rm N} - H^{\rm S}
%%& = \frac{
%%N_{S^2} \, N_\Sigma \, (\pm \xi - 2 \, N_\Sigma - \chi \, N_{S^2})
%%}{4\pi^2 \, (2 \, \chi \, N_{S^2} \, N_\Sigma + 3 \, M^2)} \ , \nn \\
%%H^{\rm N} + H^{\rm S}
%%& = 2 \, C 
%%\mp  \frac{
%%M \, N_{S^2} \, N_\Sigma \,  \xi \,( 2 \, N_\Sigma + \chi \, N_{S^2})
%%}{2\pi^2 \, (2 \, \chi \, N_{S^2} \, N_\Sigma + 3 \, M^2)}
%%\nn \\
%%&+ \frac{
%%M \, N_{S^2} \, N_\Sigma \, (8 \, N_\Sigma^2
%%+ 6 \, \chi \, N_{S^2} \, N_\Sigma + 2 \, \chi^2 \, N_{S^2}^2
%%- 3 \, M^2)
%%}{4\pi^2 \, (2 \, \chi \, N_{S^2} \, N_\Sigma + 3 \, M^2)^2}
%%\ , \nn \\
%%C_{S^2} & =
%%-2 \, C
%%- \frac 12  \, (f_{S^2}^{\rm N} + f_{S^2}^{\rm S})
%%\pm \frac{M \,  \xi \,   N_{S^2} \,  \left(2 N_{\Sigma }
%%   \left(\chi   \, N_{S^2} + 4  \,  N_{\Sigma }\right)-3 \,
%%   M^2\right)}{8 \pi ^2 \,  \left(2  \, \chi  \,  N_{S^2}
%%   N_{\Sigma } + 3  \, M^2 \right){}^2}
%%   \nn \\
%%   &+\frac{M  \, N_{S^2} \,  \left(3 \,  M^2 \, 
%%   \left(\chi \,  N_{S^2}+4\,  N_{\Sigma }\right)-2 \, 
%%   N_{\Sigma } \left(4 \, \chi \,   N_{\Sigma }  \, N_{S^2}+\chi
%%   ^2 \,  N_{S^2}^2+8  \, N_{\Sigma }^2\right)\right)}{8 \pi
%%   ^2  \, \left(2  \, \chi \,  N_{S^2} \,  N_{\Sigma
%%   }  + 3  \, M^2 \right){}^2}  \ , \nn \\
%%C_\Sigma & =    
%%-\chi \, C 
%%- \frac 12  \, (f_{\Sigma}^{\rm N} + f_{\Sigma}^{\rm S})
%%  \pm \frac{M  \, \xi \,   N_{\Sigma } \,  \left(2  \, \chi  \, 
%%   N_{S^2} \left(\chi  \,  N_{S^2}+N_{\Sigma }\right)-3 \, 
%%   M^2\right)}{8 \pi ^2 \,  \left(2  \, \chi \,   N_{S^2} \, 
%%   N_{\Sigma }  + 3 \,  M^2 \right){}^2}
%%   \nn \\
%%   & +\frac{M \, N_{\Sigma } \,  \left(3 \, 
%%   M^2 \left(\chi   \, N_{S^2}+N_{\Sigma }\right)-\chi  \, 
%%   N_{S^2}  \, \left(2 \,  \chi   \, N_{\Sigma }  \, N_{S^2}+\chi ^2 \, 
%%   N_{S^2}^2+2 \,  N_{\Sigma }^2\right)\right)}{4 \pi ^2 \, 
%%   \left(2 \, \chi \, N_{S^2}  \, N_{\Sigma
%%   } + 3 \, M^2 \right){}^2}  \ , 
%%   \nn \\
%%u & =    - C \ ,
%%\end{align}
%%where we have introduced the shorthand notation
%%\beq
%%\xi =\sqrt{
%%4 \, N_\Sigma^2 + 2 \, \chi \, N_{S^2} \,N_\Sigma + \chi^2 \, N_{S^2}^2
%%- 3 \, M^2
%%}\ . 
%%\eeq
%%The quantity $C$ is   an arbitrary constant, related to the 
%%aforementioned redundancy in our parametrization of $E_4$.
%%If we plug \eqref{good_solus} into $\int_{M_6} E_4^3$
%%we obtain the result recorded in \eqref{GMSW_result}.
%%
%%
% 
% 
%\newpage
%
%\beq
%V_2^\varphi  = \frac{V_1}{2\pi} \ , \qquad
%V_2^\Sigma = \frac{V_2}{2\pi} \, \frac \chi 2
%\eeq
%
%\beq \label{GMSW_review_flux}
%G_4 = (2\pi)^2 \, \Big[  
%2 \, d\gamma_1 \,    V_2^\varphi  \, \frac{\widehat D\psi}{2\pi}
%+ 2 \, d\gamma_2 \,   V_2^\Sigma \, \frac{
%\widehat D\psi}{2\pi}
%+ (4 \,  \gamma_2 + 4\, \gamma_1 + \frac 2 \chi \,  a_0) \,   V_{2}^\varphi \, V_{2}^\Sigma
%\Big] \ ,
%\eeq
%
%
%\beq
%d \bigg[
%(f_\varphi \, V_2^\varphi + f_\Sigma \, V_2^\Sigma) \, \frac{\widehat D \psi}{2\pi}
%\bigg]
%= (df_\varphi \, V_2^\varphi + df_\Sigma \, V_2^\Sigma) \, \frac{\widehat D \psi}{2\pi}
% - 2 \, (f_\varphi \, V_2^\varphi + f_\Sigma \, V_2^\Sigma)(V_2^\varphi + V_2^\Sigma)
%\eeq
%\beq
%d \bigg[
%(f_\varphi \, V_2^\varphi + f_\Sigma \, V_2^\Sigma) \, \frac{\widehat D \psi}{2\pi}
%\bigg]
%= (df_\varphi \, V_2^\varphi + df_\Sigma \, V_2^\Sigma) \, \frac{\widehat D \psi}{2\pi}
% - 2 \, (f_\varphi \, V_2^\varphi + f_\Sigma \, V_2^\Sigma)(V_2^\varphi + V_2^\Sigma)
%\eeq
%
%with the functions $\gamma_i$  given as
%\begin{align} \label{fi_expr}
%\gamma_1 & = \frac{
%2  \, a_2 \,  k_1 \,  k_2 \,  y+6  \, a_2 \,  f_0 +a_1 \,  y+k_1  \, y^3
%}{
%9  \, k_1 \, k_2 \,   \left(k_2 \,  y^2 -a_2\right)
%}   
%\ , \nn \\
%\gamma_2 & = \frac{
%2 \,  a_1 \,  k_1 \,  k_2 \,  y+6  \, a_1 \,  f_0 +a_2 \,  y+k_2 \,  y^3
%}{
%9 \, k_1 \, k_2 \,  \left(k_1 \, y^2-a_1\right)
%}  
%\ .
%\end{align}
%
%
%The 11d metric reads
%\begin{align} \label{GMSW_review_metric}
%ds^2_{11} & = L^2 \, e^{2\lambda} \, \Big[ ds^2(AdS_5) 
%+  ds^2(M_6) \Big] \ ,  \nn  \\
%ds^2(M_6) & = e^{-6\lambda} \Big[ F_1 \, d  s^2(C_1)
%+ F_2 \, d  s^2(C_2) \Big]
%+ \frac{e^{-6\lambda}}{\cos^2\zeta} dy^2
%+ \frac{\cos^2 \zeta}{9} D\psi^2 \ , \nn \\
%dD\psi &= \chi_1 \, V_{C_2} + \chi_2 \, V_{C_2} \ .  
%\end{align}
%The constant $L$ is the overall length scale of the solution.
%The metric on $AdS_5$ is normalized in such a way that 
%the Ricci scalar is $R_{\rm AdS_5} = -20$.
%The spaces $C_1$, $C_2$ are two Riemann surfaces, of arbitrary genus.
%If $C_i$, $i = 1,2$, is not a torus, the metric $ds^2(C_i)$
%is normalized so that the Ricci scalar is $R_{C_i}= 2 \, k_i$,
%with $k_i = \pm 1$. The symbol $\chi_i$ denotes the Euler
%characteristic of $C_i$,
%while $V_{C_i}$ is proportional to the volume form on $C_i$.
%If $C_i$ is not a torus, $V_{C_i}$ is normalized according to
%$\int_{C_i} V_{C_i}  = 2\pi$,
%with no sum over $i$.
%
%The quantities $\lambda$, $F_i$ 
%depend on $y$ only and are given by
%\begin{align}
%e^{6\lambda} &= 
%\frac{2   \left(a_1-k_1 \,  y^2\right) \left(a_2-k_2 \ 
%   y^2\right)}{a_2  \, k_1+a_1 \,  k_2+2  \, y \,  \left(k_1 \,  k_2 \,  y+ 3 \, \gamma_0
%    \right)}
%    \ , \qquad 
%F_i   = \frac 13 (a_i - k_i \,  y^2)    \ ,
%\end{align}
%where  $a_i$, $f_0$ are constants.
%The quantity $\zeta \in [0, \pi/2]$   is determined by
%\beq
%e^{3\lambda} \, \sin \zeta = 2  \, y \  \ .
%\eeq
%The $G_4$ flux takes the form
%\beq \label{GMSW_review_flux}
%G_4 = L^3 \, \Big[  
%d\gamma_1 \, V_{C_1} \, D\psi
%+ d\gamma_2 \, V_{C_2} \, D\psi
%+ (\chi_1 \, \gamma_2 + \chi_2 \, \gamma_1 + \gamma_0) \, V_{C_1} \, V_{C_2}
%\Big] \ ,
%\eeq
%with the functions $\gamma_i$  given as
%\begin{align} \label{fi_expr}
%\gamma_1 & = \frac{
%2  \, a_2 \,  k_1 \,  k_2 \,  y+6  \, a_2 \,  f_0 +a_1 \,  y+k_1  \, y^3
%}{
%9  \, k_1 \, k_2 \,   \left(k_2 \,  y^2 -a_2\right)
%}  \, \chi_1
%\ , \nn \\
%\gamma_2 & = \frac{
%2 \,  a_1 \,  k_1 \,  k_2 \,  y+6  \, a_1 \,  f_0 +a_2 \,  y+k_2 \,  y^3
%}{
%9 \, k_1 \, k_2 \,  \left(k_1 \, y^2-a_1\right)
%}  \, \chi_2 
%\ .
%\end{align}
%We are adopting conventions in which the quantization of $G_4$ flux 
%reads
%\beq \label{G4_quantization_convention}
%\int_{\cC_4} \frac{G_4}{(2\pi \ell_p)^3} \in \mathbb Z \ ,
%\eeq
%where $\cC_4$ is a 4-cycle and $\ell_p$ is the 11d Planck length.
%
%Let us stress that, in this work, we only consider GMSW
%solutions of the form \eqref{GMSW_review_metric},
%\eqref{GMSW_review_flux}
% in which none
%of the Riemann surfaces $C_i$ is a torus,
%so that $k_i \neq 0$.
%According to the analysis of \cite{Gauntlett:2004zh},
%in order to a have a regular solution 
%at least one of the two Riemann surfaces must be a sphere.
%We associate the label 1 to this sphere, 
%while the label 2 is reserved to a Riemann surface of genus $g$,
%with $g = 0$ or $g \ge 2$,
%\beq
%C_1 = S^2 \ , \qquad
%C_2 = \Sigma_g   \ .
%\eeq
%We should emphasize that the 4-form $V_4$ in \eqref{GMSW_V4}
%is understood to have integral fluxes
%along 4-cycles. It follows from \eqref{G4_quantization_convention}
%that the relation between $V_4$ and $G_4$ is
%\beq
%V_4 = \frac{G_4}{(2\pi \ell_p)^3} \ .
%\eeq 
%In the main text, we parametrized $V_4$ by writing
%\beq
%V_4 = 
%\bigg[  d\gamma_\Sigma \, \frac{V_\Sigma}{2\pi}
%+ d\gamma_{S^2} \, \frac{V_{S^2}}{2\pi} \bigg] \, \frac{D\psi}{2\pi}
%- \Big[ 2\, \gamma_\Sigma + \chi  \, \gamma_{S^2}   \Big] \,
%\frac{V_\Sigma}{2\pi}  \, \frac{V_{ S^2}}{2\pi}  \ .
%\eeq
%Comparison with \eqref{GMSW_review_flux} gives the identifications
%\beq \label{fi_identifications}
%\gamma_{S^2} = \frac{L^3}{(2\pi \ell_p)^3} \, (\gamma_1 + s_1) \ , \qquad
%\gamma_{\Sigma} = \frac{L^3}{(2\pi \ell_p)^3} \, (\gamma_2 + s_2 ) \ ,
%\qquad
%2 \, s_2 + \chi \, s_1  = \gamma_0 \ ,
%\eeq
%where the constants $s_{1,2}$ 
%can be chosen at will. In the text, 
%this ambiguity in the precise definition of $\gamma_\Sigma$, $\gamma_{S^2}$
%is resolved upon construction of $E_4$, when the condition
% \eqref{omegaI_condition} is enforced.
%
%
%\newpage
%
%
%We have presented the result in terms of
%$F^{\rm N,S}$, with $F^\mathrm C$ in \eqref{sdsds}
%considered as a dependent quantity
%
%
%
%
%The large-$N$ central charge is
%\begin{align}
%c & = \frac 98 \, \frac{N^2 (N\chi + N_{\rm N} - N_{\rm S})^2
%\, \Big[ 
%4 N^2 \chi^2 + 4 N\chi (N_{\rm N} - N_{\rm S}) 
%+ N^2_{\rm N} - 14 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%\Big]^{3/2}
%}{\Big[    4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})   \Big]^2}
%\nn \\
%& - \frac 98 \, \frac{
%N^2 (N\chi + N_{\rm N} - N_{\rm S})^2 (N_{\rm N} - N_{\rm S}) \, 
%\Big[
%N_{\rm N}^2 + 34 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%- 12 N\chi (N_{\rm N} - N_{\rm S}) - 12 N^2 \chi^2 
%\Big]
%}{\Big[    4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})   \Big]^2} \ .
%\end{align}
%
%
%We perform $a$-maximization order by order in the large-$N$
%expansion. The $\cO(N^2)$ term in $c$ turns out to be zero.
%The prediction for the $\cO(N)$ term in the central charge $c$ is
%\begin{align}
%c^{\cO (N)} &  =
%- \frac{11}{8} \, \frac{
%N\chi (N\chi + N_{\rm N} - N_{\rm S}) \,
%\Big[ 
%4 N^2 \chi^2 + 4 N\chi (N_{\rm N} - N_{\rm S}) 
%+ N^2_{\rm N} - 14 \, N_{\rm N} N_{\rm S} + N_{\rm S}^2
%\Big]^{1/2}
%}{
% 4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})  
%}
%\nn \\
%&
% - \frac 38 \,
%\frac{ (N_{\rm N} - N_{\rm S}) \, \Big[
%(N_{\rm N} + N_{\rm S})^2 + 6 N\chi (N_{\rm N} - N_{\rm S}) + 6N^2 \chi^2
%\Big]  }{
% 4N^2 \chi^2 - 3 (N_{\rm N} + N_{\rm S})^2 + 4 N\chi (N_{\rm N}
%- N_{\rm S})  
%} \ .
%\end{align}
%It is derived assuming that decoupling terms are $\cO(N^0)$,
%but otherwise arbitrary.
%
%
%
%\newpage
% The form $E_4$ is a closed and gauge invariant global angular form that encode the boundary condition of $G_4$ near the source, i.e. 
%\begin{equation}
%\mbox{near } \quad r =0  \qquad G_4 = \rho(r) E_4 + \dots
%\end{equation} where $\rho(r)$ is a bump function that smooth out the delta function at $r=0$, it vanishes as $r\to \infty$ and approach $1$ in the $r=0$ limit.  The ellipses correspond to terms that are trivial near the boundary.  
%
%The form $E_4$ is defined on the space $M_{10}$ that correspond to the boundary of the M-theory background near $r=0$.  In the case of interest, $M_{10}$ is given by the bundle
%\begin{equation}
%M_4 \hookrightarrow M_{10} \rightarrow W_6.
%\end{equation} The structure group is given by the isometry group of $M_4$.  $E_4$ is obtained by expanding on all possible globally define and gauge invariant forms on $M_{10}$ and then impose the Bianchi identity, $d E_4=0$.  In the case of interest, we can write an ansatz
%\begin{equation}
%E_4 = 2 N e_4 +F^N \omega_N +  F^S \omega_S + u_3 p_1(TW_6).  
%\end{equation} Now we explain the origin of each term.  The two-forms $(F^N= dA^N , F^S= dA^S)$ are the curvatures for the $U(1)$ gauges fields that we can turn on from blowing up the orbifold singularity.  The term $p_1(TW_6)$ is the first Pontryagin class of the tangent bundle of $W_6$.  It is closed and gauge invariant on its own, thus the parameter $u_3$ is an unfix constant.  
%
%The four-form $e_4$ is a smooth representative of the global angular form of the four-sphere with the orbifold action, it is given as
%\begin{equation}
%e_4 = \frac{1}{4\pi} \left[d\gamma(\mu) \wedge \widetilde{D} \psi + \gamma(\mu) \left( 2e_2 - F^\psi \right) \right]\wedge e_2 + u_1 e_2^2 + u_2 \left(F^\psi \right)^2. \label{e4M4}
%\end{equation} The function $\gamma(\mu)$ is constrained by regularity conditions and flux quantization, i.e.
%\begin{equation}
%N= \int_{\mathbb{R} \times \mathbb{C}^2/\mathbb{Z}_k} d G_4 \quad \Rightarrow \quad  \frac{1}{2}= \int_{S^4/\mathbb{Z}_2} e_4 =  \frac{1}{2} \left(\gamma(\mu_N)- \gamma(\mu_S)\right).   \label{intconk}
%\end{equation}
%The two-form $e_2$ is the gauge invariant global angular form for $S^2_\varphi$ given as
%\begin{equation}\label{e2svarphi}
%4\pi e_2 = D\Omega_2 + \epsilon_{abc} F^{ab} y^c, \quad \mbox{so that} \quad \int_{S^2_\varphi} e_2 =1.   
%\end{equation}  This is obtained by gauging the $SO(3)$ action of the sphere given by using embedding coordinates\footnote{\begin{equation} y^1 = \sin{\theta} \cos(\varphi), \quad y^2 = \sin(\theta) \sin(\varphi), \quad y^3 = \cos(\theta). \end{equation}} as 
%\begin{equation}
%Dy^a= dy^a + A^{ab} y^b, \qquad D\Omega_2 = \frac{1}{2} \epsilon_{abc} Dy^a Dy^b y^c.
%\end{equation}In these expressions, $(A^{ab},F^{ab})$ are respectively the $SO(3)$ connection and its curvature; they are valued on the worldvolume direction, $W_6$, of $M_{10}$.
%
%The one-form for the $\psi$ circle must be consistent with gauging of the $S^2_\varphi$,
%\begin{equation}
%\widetilde{D} \psi = d\psi + V^\varphi - A^\psi, \quad \mbox{with} \quad dV^\varphi = 2 e_2, \quad F^\varphi = d A^\varphi 
%\end{equation}  where $A^\psi$ is the gauge field associated to the $U_\psi(1)$.  
%
%The $e_2^2$ term and $(F^{\psi})^2$ term are independently closed and gauge invariant.  In the general ansatz for $E_4$, there are four parameters that are not fixed by closure alone, these are $(\gamma(\mu_N), u_1, u_2, u_3)$.  These can be fixed by imposed the equation of motion of the four-form flux in cohomology, we will return to this issue later.  
%
%The next ingredient we need is $X_8$ on the background, the tangent bundle splits as
%\begin{equation}
%TM_{11} \, \to \, TW_6 \oplus TM_4.   
%\end{equation} The first Pontryagin class the $TM_{11}$ decompose as
%\begin{align}
%p_1(TM_{11}) &= p_1^W -4 \left(c_2^\psi + c_2^\varphi \right) + p_1^N - p_1^S \\
% p_1^W &\equiv p_1(TW_6), \quad c_2^\psi \equiv c_2[SU_\psi(2)], \quad c_2^\varphi \equiv c_2[SU_\varphi(2)], \quad p_1^{N/S} \equiv p_1(T\mathbb{R}^4_{N/S}/\mathbb{Z}_2) \nonumber 
% % &-4 c_2[SU_\psi(2)]-4 c_2[SU_\varphi(2)] + p_1(T\mathbb{R}^4_N/\mathbb{Z}_2) + p_1(T\mathbb{R}^4_S/\mathbb{Z}_2).
%\end{align} We can use decomposing rules for Pontryagin classes and collect the relevant parts of $X_8$ that will appear in the anomaly 
%\begin{align}
%192 X_8 % &= p_1^2(TW_6) - 4 p_2(TW_6) + p_1(TM_4) \left[ p_1(TM_4) -2p_1(TW_6) \right] \\
%&= 8  \left(c_2^\psi + c_2^\varphi \right) \left( 2c_2^\psi +2 c_2^\varphi + p_1^W \right) -2(p_1^N - p_1^S) \left( 4c_2^\psi +4 c_2^\varphi + p_1^W \right) \\
%&-4 p_2^W + (p_1^W)^2 + \dots \nonumber 
%\end{align} After expanding $E_4^3$ and $E_4 X_8$, we find that the relevant terms that can integrated to non-zero value are
%\begin{align}
%E_4^3 &= \frac{N^3}{(2\pi)^3} \left(d\gamma \wedge \widetilde{D} \psi - \gamma F^\psi \right)^3 \wedge e_2^3 \\ &+ \frac{3N}{2\pi}  \left(d\gamma \wedge \widetilde{D} \psi - \gamma F^\psi \right)\wedge \left[(F^N)^2 \omega_N^2 + (F^S)^2 \omega_S^2 \right] \wedge e_2 + \dots \\
%192 E_4 X_8 &= \frac{N}{2\pi} d\gamma \wedge \widetilde{D} \psi \wedge e_2 \wedge\left[  (p_1^W)^2 -4 p_2^W + 8 \left(c_2^\psi + c_2^\varphi \right) \left( 2c_2^\psi +2 c_2^\varphi + p_1^W \right) \right] \\
%&+ \frac{2\gamma N}{2\pi} e_2 \wedge (p_1^N - p_1^S) \wedge \left( 4c_2^\psi +4 c_2^\varphi + p_1^W \right)+ \dots
%\end{align}
%
%%\end{comment}
%
%\begin{comment}(BOTT-CATTANEO)
%The Bott-Cattaneo formula imply
%\begin{equation}
% \int_{S^4/\mathbb{Z}_k} e_4^{2s+2} = 0, \qquad \int_{S^4/\mathbb{Z}_k} e_4^{2s+1} = \frac{2^{-2s}}{k} \left[p_2(SO(5)) \right]^s, \qquad s=0,1,2, \cdots.
%\end{equation}
%This is constructed by taking the volume and turning gauge fields valued on the worldvolume of the branes.  Since we are considering the general $S^4/\mathbb{Z}_k$ system, we work with the volume form in 
%
%\end{comment}
%
%
%
%\newpage
%
%\begin{comment}
%\subsection{In six dimensions}
%
%
%In class $\cS_k$, the 4-manifold $M_4$ fibered over the worldvolume
%of the M5-branes is the resolution of the quotient $S^4 / \mathbb Z_k$.
%Before the quotient, we can describe $S^4$ as an $S^3$ fibration
%over an interval, and use a Hopf presentation of the $S^3$,
%\beq
%ds^2(S^4) = \frac{dy^2}{1-y^2} + (1-y^2) \, \bigg[
%\frac 14 \, ds^2(S^2_\psi) + D\varphi^2 \bigg] \ , \qquad
%\varphi \sim \varphi + 2\pi \ .
%\eeq
%The angle $\psi$ is the Cartan angle of the 2-sphere which is the base
%of the Hopf fibration.
%The action of the generator of $\mathbb Z_k$ on $S^4$ is encoded in
%\beq
%(\psi , \varphi) \quad \rightarrow \quad
%(\psi , \varphi + 2 \pi/k) \ ,
%\eeq
%which means that the periodicity of $\varphi$ is effectively
%reduced to $2\pi/k$. We redefine $\varphi$ such that
%its periodicity is again $2\pi$ after the quotient.
%We get the line element
%\beq
%ds^2(S^4/\mathbb Z_k) = \frac{dy^2}{1-y^2} + (1-y^2) \, \bigg[
%\frac 14 \, ds^2(S^2_\psi) + \frac{1}{k^2} \,  D\varphi^2 \bigg] \ , \qquad
%\varphi \sim \varphi + 2\pi \ .
%\eeq
%This 4d space has two orbifold singularities at the poles $y = \pm1$,
%which both look locally like $\mathbb R^4/\mathbb Z_k$.
%The isometries of $S^2_\psi$ correspond to the $SU(2)_R$ symmetry
%of the 6d theory,
%while $U(1)_\varphi$ is a flavor symmetry.
%An additional $SU(N)_\ell \times SU(N)_r$
%flavor symmetry originates from the resolution
%of the orbifold singularities at $y = \pm 1$.
%
%
%We can describe the resolution $M_4$ of $S^4/\mathbb Z_k$
%using a local Taub-NUT metric near each pole.
%In the Taub-NUT metric, $S^1_\varphi$ is the fiber,
%while $S^1_\psi$ is part of the $\mathbb R^3$ base.
%
%In the special case $k = 2$ we can change coordinate and
%recast the Taub-NUT space in Eguchi-Hanson form.
%In the reformulation, the new circle fiber is $S^1_\psi$,
%which is fibered over a 3d space that comprises
%$S^2_\varphi$. The geometry has a bolt:
%at the ``origin'' the fiber $S^1_\psi$ shrinks,
%but the $S^2_\varphi$ in the base has a finite size.
%This bolt is identified with the resolution $\mathbb P^1$ in the Taub-NUT
%picture.
%
%The case $k = 2$ is also special from the point of view
%of the ``bulk'' of $S^4/\mathbb Z_2$.
%Indeed, because of the prefactors $1/4$ vs $1/k^2$,
%for $k = 2$ we can freely exchange the roles of $\varphi$ and $\psi$.
%This allows us to reformulate the 
% ``bulk'' of $S^4/\mathbb Z_2$
%as an $S^1_\psi$ fibration over $S^2_\varphi$. 
% 
%Combining the ``bulk'' of $S^4/\mathbb Z_2$
%with two copies of Eguchi-Hanson at each pole, we see that the space $M_4$
%has the topology
%\beq
%S^1_\psi \hookrightarrow M_4 \rightarrow [y] \times S^2_\varphi \ .
%\eeq
%The crucial observation is that the size of $S^2_\varphi$
%varies with $y$, but is never zero, which is why
%the topology is correctly captured by a direct product
%$ [y] \times S^2_\varphi$.
%
%\subsection{Harmonic 2-forms in 6d}
%
%We can model the topology of $M_4$ with a simple line element,
%\beq
%ds^2_4 = ds^2(S^2_\varphi) + \frac{dy^2}{1-y^2} + (1-y^2) \, D\psi^2 \ , \qquad
%dD\psi = p_{S^2} \, V_{S^2} \ .
%\eeq
%This metric admits
%(at least) two linearly independent harmonic forms.
%They are of the form
%\beq
%\omega =  d (H_0 \, D\psi)  \ .
%\eeq
%Coclosure of $\omega$ implies
%\beq
%H_0 = c_1 \, e^{p_{S^2} \, y} + c_2 \, e^{-p_{S^2} \, y} \ .
%\eeq
%Guess: these harmonic 2-forms are those related to the two
%resolution $\mathbb P^1$'s at the two endpoints of the $y$ interval.
%
%
%We find no extra harmonic form that is special to $k = 2$.
%Is this correct?
%
%
%\subsection{In four dimensions}
%
%
%Let us now fiber $M_4$ over a Riemann surface $\Sigma_g$,
%getting the space $M_6$.
%In order to preserve supersymmetry,
%we need to twist the Cartan of the $SU(2)_R$ symmetry,
%which is associated to the $S^1_\psi$ circle.
%We need
%\beq
%\int_{\Sigma_g} \frac{dD\psi}{2\pi} = - \chi  \ .
%\eeq
%In principle, we could also twist $S^1_{\varphi}$,
%but we do not do so.
%
%Since $S^1_\varphi$ is untwisted, the effective 
%topology of $M_6$ is of the form
%\beq
%S^1_\psi \hookrightarrow M_6 \rightarrow [y] \times S^2_\varphi  \times \Sigma_g\ .
%\eeq
%This is exactly the same topology as the GMSW solution
%
%
%\subsection{Harmonic 2-forms in 4d}
%The topology of the GMSW solution can be modelled by a simple metric,
%\beq
%ds^2_6 = ds^2(S^2_\varphi) + ds^2(\Sigma_g) + \frac{dy^2}{1-y^2} +
%(1-y^2) \, D\psi^2  \  , \qquad
%dD\psi = p_{S^2} \, V_{S^2} + p_\Sigma \, A_\Sigma \ .
%\eeq
%This metric admits
%(at least) three linearly independent harmonic forms.
%They are of the form
%\beq
%\omega = t_{S^2} \, V_{S^2} + t_\Sigma \, A_\Sigma + d (H_0 \, D\psi)  \ .
%\eeq
%This is manifestly closed. Co-closure gives a differential equation for $H_0$,
%with schematic solution
%\beq
%H_0 = c_0 + c_1 \, e^{\lambda \, y} + c_2 \, e^{- \lambda y} \ .
%\eeq
%The quantities $c_{1,2}$ are arbitrary integration constants, 
%while $c_0$ is fixed in terms of the $t$'s and the $p$'s.
%
%NB: at first it seems that we have four parameters,
%two $t$'s and $c_{1,2}$. It turns out that they yield only three
%independent 2-forms $\omega$.
%
%
%Intuition: two out of the three harmonic forms
%are inherited from those in 6d, and simply correspond to the
%flavor symmetry from the resolution $\mathbb P^1$'s.
%The third harmonic form is new, because it only appears after
%going to four dimensions.
%Probably, it is the form obtained setting $c_{1,2} = 0$,
%which is
%\beq
%\omega = p_\Sigma \, V_{S^2} - p_{S^2} \, V_{\Sigma} \ .
%\eeq
%
%
%\end{comment}


==> topmatter.tex <==
\def\check{\textbf{CHECK!}}


%\usepackage{array,setspace,mathrsfs,amsfonts,amsmath,yfonts,dsfont,bbm,colonequals,youngtab,mathabx}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}



%\usepackage{graphicx}
%\usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{hyperref}
%\usepackage[height=8.8in,width=6.45in]{geometry}
%\def\baselinestretch{1.05}

\numberwithin{equation}{section}
\newtheorem{conj}{Conjecture}
\newtheorem{thm}{Theorem}

\def\NO#1#2{{\rm NO}(#1,#2)}
\def\CB#1{$\clubsuit$ {\bf #1} $\clubsuit$}
\def\inc#1{\vcenter{\hbox{\includegraphics[scale=.25]{#1}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ceq{\colonequals}
\def\eqc{\equalscolon}
\def\eqq{\equiv}
\def\leqs{\leqslant}
\def\geqs{\geqslant}
\def\vph{\varphi}
\def\vth{\vartheta}
\def\g{\gamma}
\def\G{\Gamma}
\def\th{\theta}
\def\Th{\Theta}
\def\tpdf{\texorpdfstring}

\DeclarePairedDelimiterX\MeijerM[3]{\lparen}{\rparen}%
{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}\delimsize\vert\,#3}

\def\zeromode#1{o\left(#1\right)}

\newcommand\MeijerG[8][]{%
  G^{\,#2,#3}_{#4,#5}\MeijerM[#1]{#6}{#7}{#8}}

\WithSuffix\newcommand\MeijerG*[7]{%
  G^{\,#1,#2}_{#3,#4}\MeijerM*{#5}{#6}{#7}}


%\def\VnoH{\VV_{\cancel{\rm H}}}
\def\VH{\VV_0}
\def\VnoH{\VV_+}
\def\VSch{\mathcal{V}_{\rm Sch}}

\newcommand{\suup}{2}
\newcommand{\sudown}{1}
\def\diag{\mathop{\mathrm{diag}}\nolimits}
\def\tr{\mathop{\mathrm{tr}}\nolimits}
\def\rank{\mathop{\mathrm{rank}}\nolimits}
\def\CP{\mathbb{CP}}
\def\GL{\mathrm{GL}}
\def\SL{\mathrm{SL}}
\def\SU{\mathrm{SU}}
\def\SO{\mathrm{SO}}
\def\USp{\mathrm{USp}}
\def\UU{\mathrm{U}}
\def\PE{\mathrm{PE}}
\def\bC{\mathbb{C}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\cH{\mathcal{H}}
\def\cDI{\mathcal{DI}}
\def\cN{\mathcal{N}}
\def\cV{\mathbb{V}}
\def\fk{\mathfrak{k}}
\def\fg{\mathfrak{g}}
\def\fh{\mathfrak{h}}
\def\sN{\text{\sffamily N}}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\vev#1{\langle#1\rangle}
\def\Hyp{\mathcal{V}}
\def\half{\frac12}
\def\S{{\mathbb S}}


\def\Vir{{\rm Vir}}
\def\AD{{\rm AD}}
\def \Rf{\mf{R}}

\def \beg#1{\begin{#1}} %This is a hack for my compiler -- doesn't have any adverse effects in general
\def \be{\beg{equation}}
\def \bea{\beg{eqnarray}}
\def \eea{\end{eqnarray}}
\def \ee{\end{equation}}

\def \a{\alpha}
\def \b{\beta}
\def \D{\Delta}

\def \PE{\mathrm{P.E.}}
%\def \NO#1{\mathop{:}\nolimits\!#1\!\mathop{:}\nolimits}
\def \goodchi{\protect\raisebox{1pt}{$\chi$}}
\def \qq{\mathbbmtt{Q}\,}
\def \Qt{\wt\QQ}
\def \St{\wt\SS}
\def \Lh{\widehat{L}}
\def \Lb{\overline{L}}
\def \af{\mf{a}}
\def \df{\mf{d}}
\def \ef{\mf{e}}
\def \gf{\mf{g}}
\def \uf{\mf{u}}
\def \glf{\mf{gl}}
\def \slf{\mf{sl}}
\def \suf{\mf{su}}
\def \sof{\mf{so}}
\def \spf{\mf{sp}}
\def \psuf{\mf{psu}}
\def \uspf{\mf{usp}}
\def \ospf{\mf{osp}}
\def \of{\mf{o}}
\def \ef{\mf{e}}
\def \hhf{\mf{h}}
\def \ceq{\colonequals}
\def \bs#1{$\clubsuit${\bf #1}$\clubsuit$}
\def \restr#1#2{{\left.\kern-\nulldelimiterspace#1\vphantom{\big|}\right|_{#2}}}

\def \Poincare{Poincar\'e}

\def \ll{\lambda}

\def \ba{{\bf a}}
\def \bb{{\bf b}}
\def \bc{{\bf c}}
\def \bd{{\bf d}}

\def \bA{{\bf A}}
\def \bB{{\bf B}}
\def \bC{{\bf C}}
\def \bD{{\bf D}}
\def \bOn{{\bf 1}}
\def \bTw{{\bf 2}}
\def \bTh{{\bf 3}}
\def \bFo{{\bf 4}}
\def \bFi{{\bf 5}}
\def \cd{{\tilde c}}

\def \hf{\frac12}
\def \qt{\frac14}

\def \mf{\mathfrak}
\def \lb{\lbrack}
\def \rb{\rbrack}
\def \nn{\nonumber}
\def \ph{\phantom}
\def \wt{\widetilde}
\def \wh{\widehat}
\def \ol{\overline}
\def \eg{{\it e.g.}}
\def \ie{{\it i.e.}}
\def \cf{{\it cf.}}
\def \Tr{{\rm Tr}}
\def \STr{{\rm STr}}
\def \til{\tilde}
\def \pr{\prime}
\def \zb{{\bar z}}
\def \db{\ol{\partial}}
\def \d{\partial}
\def \dag{\dagger}

\def \Ab{\mathbb{A}}
\def \Cb{\mathbb{C}}
\def \Eb{\mathbb{E}}
\def \Fb{\mathbb{F}}
\def \Hb{\mathbb{H}}
\def \Kb{\mathbb{K}}
\def \Mb{\mathbb{M}}
\def \Nb{\mathbb{N}}
\def \Ob{\mathbb{O}}
\def \Qb{\mathbb{Q}}
\def \Rb{\mathbb{R}}
\def \Sb{\mathbb{S}}
\def \Zb{\mathbb{Z}}


\def \AA{\mathcal{A}}
\def \BB{\mathcal{B}}
\def \CC{\mathcal{C}}
\def \DD{\mathcal{D}}
\def \EE{\mathcal{E}}
\def \FF{\mathcal{F}}
\def \GG{\mathcal{G}}
\def \HH{\mathcal{H}}
\def \II{\mathcal{I}}
\def \JJ{\mathcal{J}}
\def \KK{\mathcal{K}}
\def \LL{\mathcal{L}}
\def \MM{\mathcal{M}}
\def \NN{\mathcal{N}}
\def \OO{\mathcal{O}}
\def \PP{\mathcal{P}}
\def \QQ{\mathcal{Q}}
\def \RR{\mathcal{R}}
\def \SS{\mathcal{S}}
\def \TT{\mathcal{T}}
\def \UU{\mathcal{U}}
\def \VV{\mathcal{V}}
\def \WW{\mathcal{W}}
\def \XX{\mathcal{X}}
\def \YY{\mathcal{Y}}
\def \ZZ{\mathcal{Z}}


\def \RRR{\mathfrak{R}}

